Learning of Structurally Unambiguous Probabilistic Grammars

The problem of identifying a probabilistic context free grammar has two aspects: the first is determining the grammar's topology (the rules of the grammar) and the second is estimating probabilistic weights for each rule. Given the hardness results for learning context-free grammars in general, and probabilistic grammars in particular, most of the literature has concentrated on the second problem. In this work we address the first problem. We restrict attention to structurally unambiguous weighted context-free grammars (SUWCFG) and provide a query learning algorithm for \structurally unambiguous probabilistic context-free grammars (SUPCFG). We show that SUWCFG can be represented using \emph{co-linear multiplicity tree automata} (CMTA), and provide a polynomial learning algorithm that learns CMTAs. We show that the learned CMTA can be converted into a probabilistic grammar, thus providing a complete algorithm for learning a structurally unambiguous probabilistic context free grammar (both the grammar topology and the probabilistic weights) using structured membership queries and structured equivalence queries. A summarized version of this work was published at AAAI 21.

==> algorithms_src.tex <==
\clearpage
	\begin{algorithm}
		\caption{$\LearnCMTA(T,C,H,B)$.}\label{alg:cstar}\label{alg:learn}
		\begin{algorithmic}[1]
			\State  Initialize $B\gets\emptyset,~T\gets\emptyset,~C\gets\{\context\}$ 
			\State $\Complete(T,C,H,B,\Sigma_0)$			
			\While{true}
			\State $\mathcal{A}\gets \ExtractCMTA(T,C,H,B)$
			\State $t\gets\seq(\mathcal{A})$
			\If{$t$ is null}
			\State \Return $\mathcal{A}$
			\EndIf
			\State $\Complete(T,C,H,B,  \pref(t))$
			\EndWhile
		\end{algorithmic}
	\end{algorithm}
\clearpage
{
	\begin{algorithm}
		\caption{$\Close(T,C,H,B)$.}\label{proc:close}
		\begin{algorithmic}[1]
			\While{$\exists t\in \Sigma(T)$ s.t. $H[t]$ is co-linearly independent from $T$}
			\State $B\gets B\cup \{t\}$
			\State $T\gets T\cup \{t\}$
			\EndWhile
		\end{algorithmic}
	\end{algorithm}
}
\clearpage
{
	\begin{algorithm}
		\caption{$\Consistent(T,C,H,B)$}\label{proc:consistent}
		\begin{algorithmic}[1]
			\For{$t\in T$ s.t. $H[t]=\overline{0}$}
			\For{$c\in\Sigma(T,\context),c'\in C$}
			\If{$H[\contextConcat{c'}{c[t]}]\neq \overline{0}$}
			\State $C\gets C \cup\{\contextConcat{c}{c'}\}$
			\EndIf
			\EndFor
			\EndFor
			\For{$t_1,t_2\in T$ s.t. $ t_1\treesColin{\alpha}{H} t_2$}
			\For{$c\in\Sigma(T,\context),c'\in C$}
			\If{$H[{c'}][\contextConcat{c}{t_1}]\neq \alpha H[{c'}][{\contextConcat{c}{t_2}}]$}
			\State $C\gets C \cup\{\contextConcat{c}{c'}\}$
			\EndIf
			\EndFor
			\EndFor
		\end{algorithmic}
	\end{algorithm}
}
\clearpage
{
	\begin{algorithm}
		\caption{$\Complete(T,C,H,B,S)$.}\label{proc:complete}
		\begin{algorithmic}[1]
			\State  $T\gets T \cup S$ 
			\While{$(T,C,H,B)$ is not closed or not consistent}
			\State $\Close(T,C,H,B)$
			\State $\Consistent(T,C,H,B)$
			\EndWhile
		\end{algorithmic}
	\end{algorithm}
} 


\clearpage

\commentout{
	\begin{algorithm}
		\caption{$\Consistent(T,C,H,B)$}\label{proc:consistent}
		\begin{algorithmic}[1]
			\For{$t\in T$ s.t. $H[t]=\overline{0}$}
			\For{$t'\in\Sigma(T,t)$}
			\For{$c\in C$}
			\If{$H[\contextConcat{c}{t'}]\neq \overline{0}$}
			\State $C\gets C \cup\{\contextConcat{c}{c_t'}\}$
			\EndIf
			\EndFor
			\EndFor
			\EndFor
			\For{$t_1,t_2\in T$ s.t. $ t_1\treesColin{\alpha}{H} t_2$}
			\For{$c\in\Sigma(T,\context),c'\in C$}
			\If{$H[{c'}][\contextConcat{c}{t_1}]\neq \alpha H[{c'}][{\contextConcat{c}{t_2}}]$}
			\State $C\gets C \cup\{\contextConcat{c}{c'}\}$
			\EndIf
			\EndFor
			\EndFor
		\end{algorithmic}
	\end{algorithm}
}

\clearpage


\clearpage 

\begin{algorithm}[H]\label{alg:cstarExtract}
\caption{Extract CMTA}
\begin{algorithmic}[1]
\State $d\gets |B|$
\For {$0\leq k\leq p$}
\For {$\sigma\in \Sigma_{k}$}
\For {$(i_{1},i_{2},\dots,i_{k})\in \{1,2,\dots,d\}^{k}$}
\State Let $t=\sigma(b_{i_{1}},b_{i_{2}},\dots,b_{i_{k}})$
\If {$H[t]=\bar{0}$}
\For {$1\leq j\leq d$}
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets 0$
\EndFor
\Else
\State Let $b_{i}\in B,\alpha\in\mathbb{R}$ be s.t. $t\treesColin{\alpha}{H} b_{i}$
\For {$1\leq j\leq d$}
\If {$j=i$}
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets\alpha$
\Else
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets 0$
\EndIf
\EndFor
\EndIf
\EndFor
\State Let $\mu_{\sigma}$ be the $d\times d^{k}$ matrix obtained from the respective coefficients.
\EndFor
\EndFor
\For {$1\leq j\leq d$}
\State $\lambda[j]\gets H(b_{j}, \context)$
\EndFor
\State \Return $\mathcal{A}=(\Sigma,\mathbb{R},d,\mu,\lambda)$
\end{algorithmic}
\end{algorithm}

\clearpage

\begin{figure}
\centering
	\scalebox{.9}{\small{
	\begin{tabular}{l@{\qquad\qquad}l}
$M_\eta = \begin{pmatrix}
c^1_{{111}} & c^1_{{112}}& c^1_{{121}} & c^1_{{122}} & c^1_{{211}} & c^1_{{212}}& c^1_{{221}} & c^1_{{222}} \\[1mm]
c^2_{{111}} & c^2_{{112}}& c^2_{{121}} & c^2_{{122}} & c^2_{{211}} & c^2_{{212}}& c^2_{{221}} & c^2_{{222}} 
\end{pmatrix}$
&
$P_{xyz} =  \begin{pmatrix}
x_1 y_1 z_1 \\
x_1 y_1 z_2 \\
x_1 y_2 z_1 \\
%x_1 y_2 z_2 \\
%x_2 y_1 z_1 \\
%x_2 y_1 z_2 \\
%x_2 y_2 z_1 \\
\ldots \\
x_2 y_2 z_2 \\
\end{pmatrix}$
\end{tabular}
}}\vspace{-2mm}
\end{figure} 
\clearpage
	\begin{tabular}{c@{\ \ \ }c@{\  }c}
	            \raisebox{1.0\height}{
	            \begin{tabular}{@{}c@{}}
	            \raisebox{0.9\height}{
				$\lambda=\begin{pmatrix}1\\0
				\end{pmatrix}$ 
				$\mu_{a}= \begin{pmatrix}1\\1
				\end{pmatrix}$ }
				\\[4mm]
	            $\mu_{b} = \begin{pmatrix}
				0 & 1 & 1 & 0 \\[1mm]
				0 & 0 & 0 & 1 
				\end{pmatrix}$
	            \end{tabular}}&
				\begin{tikzpicture}
				\tikzstyle{myarrow}=[line width=.5mm,draw=#1,-triangle 45,postaction={draw, line width=4mm, shorten >=5mm, -}]
				\node[shape=circle, draw=none] (a1) at (2, 1) {$a$};
				\node[] (a1v) at (3.5, 1) {${\biword{1}{1}}$};
				\node[] (a2v) at (1.5, 1) {${\biword{1}{1}}$};
				\node[shape=circle, draw=none]  (a2) at (3, 1) {$a$};
				\node[shape=circle, draw=none] (a3) at (3.65, 2.0) {$a$};
				\node[] (a3v) at (4.10, 2.0) {${\biword{1}{1}}$};
				\node[shape=circle, draw=none]  (b1) at (2.5, 2.0) {$b$};
				\node[] (a3v) at (2.0, 2.0) {${\biword{2}{1}}$};
				\node[shape=circle, draw=none]  (b2) at (3, 3) {$b$};
				\node[] (b2v) at (2.5, 3) {${\biword{3}{1}}$};
				\draw (b2) -- (a3);
				\draw (b2) -- (b1);
				\draw (b1) -- (a1);
				\draw (b1) -- (a2);
				\end{tikzpicture}&
				\raisebox{0.75\height}{
				\scalebox{1}{
				\begin{tabular}{@{}c@{}}
				\begin{tikzpicture}
				\tikzstyle{myarrow}=[line width=.5mm,draw=#1,-triangle 45,postaction={draw, line width=4mm, shorten >=5mm, -}]
				\node[shape=circle, draw=none] (a1) at (0.6, 1.46) {$a$};
				\node[shape=circle, draw=none]  (a2) at (1.6, 1.46) {$b$};
				\node[shape=circle, draw=none] (a3) at (2.25, 2.13) {$c$};
				\node[shape=circle, draw=none]  (b1) at (1.1, 2.13) {$d$};
				\node[shape=circle, draw=none]  (b2) at (1.6, 2.8) {$e$};
				\draw (b2) -- (a3);
				\draw (b2) -- (b1);
				\draw (b1) -- (a1);
				\draw (b1) -- (a2);
				%\end{tikzpicture}\\
				%\begin{tikzpicture}
				%\tikzstyle{myarrow}=[line width=.5mm,draw=#1,-triangle 45,postaction={draw, line width=4mm, shorten >=5mm, -}]
				\node[shape=circle, draw=none] (a1) at (2.2, 0.66) {$a$};
				\node[shape=circle, draw=none]  (a2) at (3.2, 0.66) {$b$};
				\node[shape=circle, draw=none] (a3) at (3.85, 1.33) {$c$};
				\node[shape=circle, draw=none]  (b1) at (2.7, 1.33) {$?$};
				\node[shape=circle, draw=none]  (b2) at (3.2, 2) {$?$};
				\draw (b2) -- (a3);
				\draw (b2) -- (b1);
				\draw (b1) -- (a1);
				\draw (b1) -- (a2);
				\end{tikzpicture}
				\end{tabular}}}
				\\
				(I.i)&(I.ii)&(II)
	\end{tabular}
\clearpage
\newcommand{\startprod}[1]{$#1\rightarrow$}
\newcommand{\derivation}[3]{\hlc[yellow!#3]{#1 [#2]}$\:\mid\:$}
\newcommand{\lastderivation}[3]{\hlc[yellow!#3]{#1 [#2]}}
\newcommand{\spacing}[0]{\:}
\newcommand{\cfgopt}[0]{\,|\,}
\newcommand{\scalefactor}{0.9}
\newcommand{\hlc}[2][yellow]{{%
    \colorlet{foo}{#1}%
    \sethlcolor{foo}\hl{#2}}%
}
\scalebox{\scalefactor}{
\:\:\:\startprod{S} \makebox[8.45cm]{\derivation{R N7}{0.456}{45}\derivation{R N3}{0.185}{18}\derivation{C N1}{0.137}{13}\derivation{N7 R}{0.078}{7}}
}
\scalebox{\scalefactor}{
\makebox[11.25cm]{\derivation{R N6}{0.053}{5}\derivation{N1 C}{0.034}{3}\derivation{N5 R}{0.028}{2}\derivation{N6 R}{0.013}{1}}
}
\scalebox{\scalefactor}{
\makebox[6.72cm]{\derivation{N3 R}{0.012}{1}\lastderivation{R N5}{0.004}{0}}
}

\scalebox{\scalefactor}{
\startprod{N1} \derivation{R N2}{0.640}{64}\derivation{N2 R}{0.160}{16}\derivation{R N4}{0.160}{16}\lastderivation{N4 R}{0.040}{4}
}

\scalebox{\scalefactor}{
\startprod{N2} \lastderivation{A B}{1.000}{100} \startprod{N3} \lastderivation{C N2}{1.000}{100}  \startprod{N4} \lastderivation{B A}{1.000}{100}
}

\scalebox{\scalefactor}{
\startprod{N5} \lastderivation{N4 C}{1.000}{100} \startprod{N6} \derivation{C N4}{0.882}{88}\derivation{N8 A}{0.095}{9}\lastderivation{A N8}{0.024}{2}
}

\scalebox{\scalefactor}{
\startprod{N7} \lastderivation{N2 C}{1.000}{100} \startprod{N8} \derivation{B C}{0.800}{80}\lastderivation{C B}{0.200}{20}
}

\scalebox{\scalefactor}{
\:\:\:\startprod{R} \lastderivation{AcrR}{1.000}{100} \startprod{A} \lastderivation{AcrA}{1.000}{100} \startprod{B} \lastderivation{AcrB}{1.000}{100}
}

\scalebox{\scalefactor}{
\:\:\:\startprod{C} \lastderivation{TolC}{1.000}{100}
}

\begin{tikzpicture}
\node[draw=none] (t1) at (0, 0) {
\scalebox{0.6}{
\begin{tikzpicture}
\tikzstyle{myarrow}=[line width=3mm,draw=#1]
\draw [myarrow={cyan}](1.2,3.5)--(-0,3.5);
\draw [myarrow={red}](1.4,3.5)--(2.6,3.5);
\draw [myarrow={green}](3,3.5)--(4.2,3.5); 
\draw [myarrow={yellow}](4.5,3.5)--(5.7,3.5); 
\node[draw=none] (S) at (2.5, 6) {$S$};
\node[draw=none] (R) at (0.6, 5) {$R$};
\node[draw=none] (A) at (2, 4.25) {$A$};
\node[draw=none] (B) at (3.5, 4.25) {$B$};
\node[draw=none] (C) at (5, 4.25) {$C$};
\node[draw=none] (N2) at (2.7, 5) {$N_{2}$};
\node[draw=none] (N7) at (3.7, 5.5) {$N_{7}$};
\node[draw=none] (acrA) at (2,3.5) {AcrA};
\node[draw=none] (acrB) at (3.5,3.5) {AcrB};
\node[draw=none] (tolC) at (5,3.5) {TolC};
\node[draw=none] (acrR) at (0.6,3.5) {AcrR};
\draw (S) -- (N7);
\draw (S) -- (R);
\draw (N7) -- (N2);
\draw (N7) -- (C);
\draw (N2) -- (A);
\draw (N2) -- (B);
\draw (R) -- (acrR);
\draw (A) -- (acrA);
\draw (B) -- (acrB);
\draw (C) -- (tolC);
\end{tikzpicture}}};
\node[draw=none] (t2) at (5, 0) {\scalebox{0.6}{
\begin{tikzpicture}
\tikzstyle{myarrow}=[line width=3mm,draw=#1]
\draw [myarrow={cyan}](3,3.75)--(4.2,3.75); 
\draw [myarrow={red}](1.4,3.75)--(2.6,3.75);
\draw [myarrow={green}](1.2,3.75)--(-0,3.75);
\draw [myarrow={yellow}](4.5,3.75)--(5.7,3.75); 
\node[draw=none] (S) at (3.5, 6.3) {$S$};
%\node[draw=none] (Ps) at (3.5, 7) {$0.522$}
\node[draw=none] (N1) at (2.5, 5.75) {$N_{1}$};
%\node[draw=none] (P1) at (0.5, 4.5) {$1.000$}
\node[draw=none] (A) at (2, 4.5) {$A$};
%\node[draw=none] (P2) at (2.2, 3.25) {$1.000$}
\node[draw=none] (B) at (0.5, 4.5) {$B$};
\node[draw=none] (R) at (3.5, 5) {$R$};
%\node[draw=none] (P3) at (4.2, 3.25) {$1.000$}
\node[draw=none] (N4) at (1.25, 5) {$N_{4}$};
\node[draw=none] (C) at (5, 5) {$C$};
\node[draw=none] (acrA) at (2,3.75) {AcrA};
\node[draw=none] (acrB) at (0.5,3.75) {AcrB};
\node[draw=none] (tolC) at (5,3.75) {TolC};
\node[draw=none] (acrR) at (3.5,3.75) {AcrR};

\draw (S) -- (N1);
\draw (S) -- (C);
\draw (N1) -- (N4);
\draw (N1) -- (R);
\draw (N4) -- (B);
\draw (N4) -- (A);
\draw (R) -- (acrR);
\draw (A) -- (acrA);
\draw (B) -- (acrB);
\draw (C) -- (tolC);
\end{tikzpicture}}};

\node[draw=none] (t3) at (2.5,0.2) {\scalebox{0.55}{\begin{tikzpicture}
\tikzstyle{myarrow}=[line width=3mm,draw=#1]
\draw [myarrow={cyan}](1,1.5)--(1,2.5);
\draw [myarrow={red}](0,1.5)--(0,2.5);
\draw [myarrow={green}](2,1.5)--(2,2.5);
\draw [myarrow={yellow}](3,1.5)--(3,2.5); 
\node[shape=circle,draw=black] (P) at (1.5, 3.5) {};
\node[draw=none, rotate=90] (acrA) at (0,2) {AcrA};
\node[draw=none, rotate=90] (acrB) at (2,2) {AcrB};
\node[draw=none, rotate=90] (tolC) at (3,2) {TolC};
\node[draw=none, rotate=90] (acrR) at (1,2) {AcrR};

\draw (P) -- (acrR);
\draw (P) -- (acrA);
\draw (P) -- (acrB);
\draw (P) -- (tolC);
\end{tikzpicture}}};
\end{tikzpicture}

==> learningSUPCFG.tex <==
To overcome the issues with learning a general PCFG, we restrict attention to structurally unambiguous CFGs (SUCFGs), as defined shortly, and their weighted/probabilistic versions (SUWCFGs/SUPCFGs).
\subsection{Structurally Unambiguous Grammars}\label{sec:sucfg}
\begin{defi}
A CFG $\mathcal{G}$ is structurally unambiguous (SUCFG) iff for every two derivation trees $t_{1},t_{2}$ derived from the grammar $\skel(t_{1})=\skel(t_{2})$ implies that $t_{1}=t_{2}$.
\end{defi}
Figure \ref{fig:ucfg} depicts a structurally ambiguous grammar, with the two parse trees that cause the structural ambiguity.
\begin{figure}
    \centering
    \begin{minipage}{\textwidth}
        \begin{align*}
            S&\rightarrow N_{1}b\mid N_{2}b\\
            N_{1}&\rightarrow aa\\
            N_{2}&\rightarrow aa
        \end{align*}
    \end{minipage}
    \begin{minipage}{0.33\textwidth}
        \begin{tikzpicture}
    	\foreach \i\j\n\label in {0/0/A/$S$,-1/-1/B/$N_{1}$,1/-1/C/$b$, -2/-2/D/$a$,0/-2/E/$a$}{
        	\node[shape=circle,draw=none] (\n) at (\i,\j) {\tiny{\label}};
    	}
        \path [-] (A) edge node[above] {} (C);
        \path [-] (A) edge node[right] {} (B);
        \path [-] (B) edge node[right] {} (D);
        \path [-] (B) edge node[right] {} (E);
        \end{tikzpicture}
    \end{minipage}%
    \begin{minipage}{0.33\textwidth}
        \begin{tikzpicture}
    	\foreach \i\j\n\label in {0/0/A/$S$,-1/-1/B/$N_{2}$,1/-1/C/$b$, -2/-2/D/$a$,0/-2/E/$a$}{
        	\node[shape=circle,draw=none] (\n) at (\i,\j) {\tiny{\label}};
    	}
        \path [-] (A) edge node[above] {} (C);
        \path [-] (A) edge node[right] {} (B);
        \path [-] (B) edge node[right] {} (D);
        \path [-] (B) edge node[right] {} (E);
        \end{tikzpicture}
    \end{minipage}%
    \begin{minipage}{0.33\textwidth}
        \begin{tikzpicture}
    	\foreach \i\j\n\label in {0/0/A/$?$,-1/-1/B/$?$,1/-1/C/$b$, -2/-2/D/$a$,0/-2/E/$a$}{
        	\node[shape=circle,draw=none] (\n) at (\i,\j) {\tiny{\label}};
    	}
        \path [-] (A) edge node[above] {} (C);
        \path [-] (A) edge node[right] {} (B);
        \path [-] (B) edge node[right] {} (D);
        \path [-] (B) edge node[right] {} (E);
        \end{tikzpicture}
    \end{minipage}%

    \caption{A structurally ambiguous grammar $\mathcal{G}$ (top), with its two parse trees (left and middle), that share the same structural description (right).}
    \label{fig:ucfg}
\end{figure}
\subsection{Colinear Multiplicity Tree Automata}\label{sec:cmta}
\begin{defi}
A Multiplicity Tree Automaton is termed \emph{colinear} if for every $\sigma\in\Sigma$, the matrix representing the multilinear transformation $\mu_{\sigma}$ has at most a single non-zero entry in each column.
\end{defi}
We use CMTA to refer to colinear multiplicity tree automata.
\begin{exa}
The following MTA $M$ isn't a colinear one, since $M_{\mu_{a}}$ has a column with two non-zero entries.
\vspace{0.2cm}
\begin{equation}
    M=\langle R^{2},\Sigma=\{\Sigma_{2}=\{b\},\Sigma_{0}=\{a\}\},\lambda,\mu\rangle
\end{equation}
\begin{minipage}{0.33\textwidth}
    \begin{equation*}
        M_{\mu_{a}}=\begin{bmatrix}&\cellcolor{gray!10}1&\\&\cellcolor{gray!10}1&\end{bmatrix}
    \end{equation*}
\end{minipage}%
\begin{minipage}{0.33\textwidth}
\vspace{-0.5cm}
    \begin{equation*}
        M_{\mu_{b}}=\begin{bmatrix}&0&1&1&0&\\
                                   &0&0&0&1&\end{bmatrix}        
    \end{equation*}

\end{minipage}%
\begin{minipage}{0.33\textwidth}
    \begin{equation*}
        \lambda=\begin{bmatrix}&1&\\&0&\end{bmatrix}        
    \end{equation*}

\end{minipage}
\vspace{0.25cm}

But the MTA $N$, below, is colinear, since in every matrix, each column has at most a single non-zero entry:
\vspace{0.2cm}
\begin{equation}\label{CMTAExample}
    N=\langle R^{2},\Sigma=\{\Sigma_{2}=\{b\},\Sigma_{0}=\{a\}\},\lambda,\mu\rangle
\end{equation}
\begin{minipage}{0.33\textwidth}
    \begin{equation*}
        M_{\mu_{a}}=\begin{bmatrix}&1&\\&0&\end{bmatrix}
    \end{equation*}
\end{minipage}%
\begin{minipage}{0.33\textwidth}
\vspace{-0.5cm}
    \begin{equation*}
        M_{\mu_{b}}=\begin{bmatrix}&0&0&0&0&\\
                                   &\frac{1}{2}&0&0&\frac{1}{2}&\end{bmatrix}        
    \end{equation*}

\end{minipage}%
\begin{minipage}{0.33\textwidth}
    \begin{equation*}
        \lambda=\begin{bmatrix}&0&\\&1&\end{bmatrix}        
    \end{equation*}

\end{minipage}
\end{exa}
\subsubsection{The Hankel Matrix of a CMTA}
\begin{defi}
Two vectors $v_{1},v_{2}$ are colinear iff $v_{1}=\alpha\cdot v_{2}$, for some $\alpha\neq 0$.
\end{defi}
\begin{defi}
Let $L$ be some tree-series, and let $H$ be the Hankel Matrix for that tree series. Let $t_{1},t_{2}$ be two trees. We say that $t_{1}$ and $t_{2}$ are colinear with coefficient $\alpha\neq 0$ with respect to $H$, denoted by $t_{1}\treesColin{\alpha}{H} t_{2}$, iff $H[t_{1}]=\alpha\cdot H[t_{2}]$. That is, for every context $c$ we have:
\begin{equation*}
L(\contextConcat{c}{t_{1}})=\alpha\cdot L(\contextConcat{c}{t_{2}})
\end{equation*}
\end{defi}
Using these definitions, we can define a relation on $\trees(\Sigma)$, s.t. $t_{1}\sim_{H} t_{2}$ iff there exists some $\alpha>0$ s.t. $t_{1}\treesColin{\alpha}{H} t_{2}$. One can observe that $\sim_{H}$ is an equivalence relation, we will denote it from now by $\equiv_{H}$. We will now show that if $H$ is the Hankel Matrix of a language generated by a CMTA, then $\equiv_{H}$ has a finite number of equivalence classes.
\begin{lem}\label{lemma:oneHotVec}
    Let $\mathcal{A}=\langle\mathbb{F}^{d},\Sigma,\lambda,\mu\rangle$ be a CMTA. For every $t\in\trees(\Sigma)$ we have that $\mu(t)$ has at most a single non-zero entry.
\end{lem}
\begin{proof}
    For brevity, since the matrix $\mu_{\sigma}$ has $d^{p}$ columns, and the vector $P_{v_{1}v_{2}\dots v_{p}}$ is of size $d^{p}$, we will denote by $\mu_{\sigma}[i_{1},i_{2},\dots,i_{p}]$ (resp. $P_{v_{1}v_{2}\dots v_{p}}[i_{1},i_{2},\dots,i_{p}]$) the column vector (resp. entry) in the matrix (resp. vector) that corresponds to the product of $v_{1}[i_{1}]\cdot v_{2}[i_{2}]\cdot \dots \cdot v_{p}[i_{p}]$, that is: 
    \begin{equation*}
        \mu_{\sigma}[i_{1},i_{2},\dots,i_{p}] = \mu_{\sigma}[\sum_{j=1}^{p} i_{j}\cdot d^{p-j+1}]
    \end{equation*}
    \begin{equation*}
        P_{v_{1}v_{2}\dots v_{p}}[i_{1},i_{2},\dots,i_{p}] = P_{v_{1}v_{2}\dots v_{p}}[\sum_{j=1}^{p} i_{j}\cdot d^{p-j+1}]
    \end{equation*}
    We will prove by induction on the height of $t$.
    
    \textbf{Base case:} The height of $t=\sigma$ is $1$, and $t$ is a leaf, then $\mu(t)=\mu_{\sigma}()$. By definition of a CMTA, $\mu_{\sigma}()$ has at most a single non-zero entry.
    
    \textbf{Induction step:} The height of $t$ is $h>1$, then $t=\sigma(t_{1},t_{2},\dots,t_{p})$. For each $i$ the height of $t_{i}$ is at most $h-1$, so by our induction hypothesis, $\mu(t_{i})$ has at most a single non-zero entry. If for some $i$ $\mu(t_{i})=\bar{0}$ then $P_{\mu(t_{1})\mu(t_{2})\dots\mu(t_{p})}=\bar{0}$. Let's assume that for every $i$, there exists $j_{i}$ s.t. $\mu(t_{i})[j_{i}]\neq 0$. Then $P_{\mu(t_{1})\mu(t_{2})\dots\mu(t_{p})}$ has exactly a single non-zero entry, the one corresponding to: $\prod_{i=1}^{p} \mu(t_{i})[j_{i}]$.  Since $\mathcal{A}$ is a CMTA, the column of the matrix $\mu_{\sigma}$ which corresponds to the indices $(j_{1},j_{2},\dots,j_{p})$ has at-most a single non-zero entry. So $\mu_{\sigma}[i][j_{1},j_{2},\dots,j_{p}]=\alpha$ and for every $j\neq i$ we have $\mu_{\sigma}[i][j_{1},j_{2},\dots,j_{p}]=0$.
    
    By definition, $\mu(t)=\mu_{\sigma}\cdot P_{\mu(t_{1})\mu(t_{2})\dots\mu(t_{p})}$, for every $j\neq i$, we have:
    \begin{align*}
        \mu(t)[j]&=\sum_{i_{1},i_{2},\dots,i_{p}} P_{\mu(t_{1})\mu(t_{2})\dots\mu(t_{p})}[i_{1},i_{2},\dots,i_{p}]\cdot \mu_{\sigma}[j][i_{1},i_{2},\dots,i_{p}]\\
        &=\sum_{i_{1},i_{2},\dots,i_{p}} 0\cdot \mu_{\sigma}[j][i_{1},i_{2},\dots,i_{p}]=0
    \end{align*}
    For $i$ we have:
    \begin{align*}
        \mu(t)[i]&=\sum_{i_{1},i_{2},\dots,i_{p}} P_{\mu(t_{1})\mu(t_{2})\dots\mu(t_{p})}[i_{1},i_{2},\dots,i_{p}]\cdot \mu_{\sigma}[i][i_{1},i_{2},\dots,i_{p}]\\
        &=\alpha\cdot P_{\mu(t_{1})\mu(t_{2})\dots\mu(t_{p})}[j_{1},j_{2},\dots,j_{p}]
    \end{align*}
    As required.
\end{proof}
\begin{lem}\label{lemma:contextMaintainsOneHot}
    Let $t_{1},t_{2}$ be two trees s.t. $\mu(t_{1})=\alpha_{1}\cdot v_{i}\neq\bar{0}$ and $\mu(t_{2})=\alpha_{2}\cdot v_{i}\neq\bar{0}$. The for every context $c$ we have that:
        \begin{equation*}
            H[t_{1}][c]=\frac{\alpha_{2}}{\alpha_{1}} H[t_{2}][c]
        \end{equation*}
\end{lem}
\begin{proof}
    Let $c$ be a context, we will prove by induction on the depth of $\context$ in $c$.
    
    \textbf{Base case:} The depth of $\context$ in $c$ is $0$, so $c=\context$. Then $\contextConcat{c}{t_{1}}=t_{1}$ and $\contextConcat{c}{t_{2}}=t_{2}$. We have that $H[t_{1}][c]=\alpha_{1}\cdot v_{i}\cdot\lambda^{\top}$ and that $H[t_{2}][c]=\alpha_{2}\cdot v_{i}\cdot\lambda^{\top}$. $v_{i}\cdot\lambda^{\top}$ is some scalar, so:
    \begin{equation*}
        H[t_{1}][c]=\frac{\alpha_{2}}{\alpha_{1}} H[t_{2}][c]
    \end{equation*}
    
    \textbf{Induction step:} The depth of $\context$ in $c$ is $h+1$ for $h\geq 0$. We assume that the claim holds for all contexts s.t. the depth of $\context$ in $c$ is at most $h$. Since the depth of $\context$ in $c$ is at least $1$, we have that:
    \begin{equation*}
        c=\contextConcat{c'}{\sigma(m_{1},m_{2},\dots,m_{l-1},\context,m_{l+1},\dots,m_{p})}
    \end{equation*}
    For some context $c'$ s.t. the depth of $\context$ in $c'$ is $h$. We will first show that
    \begin{equation*}
        \mu(\sigma(m_{1},m_{2},\dots,m_{l-1},t_{1},m_{l+1},\dots,m_{p}))=\frac{\alpha_{2}}{\alpha_{1}}\cdot\mu(\sigma(m_{1},m_{2},\dots,m_{l-1},t_{2},m_{l+1},\dots,m_{p}))
    \end{equation*}
    By Lemma \ref{lemma:oneHotVec} we have that for every $1\leq k\neq l \leq p$ $\mu(m_{r})$ has at most a single non-zero entry. We will denote $\mu(m_{r})$ by $\alpha_{r}\cdot v_{j_{r}}$, where $v_{j_{r}}$ is the $j_{r}$'th standard basis vector. We can now obtain: 
    \begin{align*}
        P_{\mu(m_{1})\mu(m_{2})\dots\mu(m_{i-1})\mu(t_{1})\mu(m_{i+1})\dots\mu(m_{p})}[j_{1},j_{2},\dots,j_{l-1},i,j_{l+1},\dots,j_{p}]&=\alpha_{1}\cdot\prod_{r=1}^{p}\alpha_{r}\\
        P_{\mu(m_{1})\mu(m_{2})\dots\mu(m_{i-1})\mu(t_{2})\mu(m_{i+1})\dots\mu(m_{p})}[j_{1},j_{2},\dots,j_{l-1},i,j_{l+1},\dots,j_{p}]&=\alpha_{2}\cdot\prod_{r=1}^{p}\alpha_{r}        
    \end{align*}
    And for every other indices, $P_{\mu(m_{1})\mu(m_{2})\dots\mu(m_{l-1})\mu(t_{s})\mu(m_{l+1})\dots\mu(m_{p})}[i_{1},i_{2},\dots,i_{p}]=0$.
    Then we can obtain that:
    \begin{equation*}
        \mu_{\sigma}\cdot P_{\mu(m_{1})\mu(m_{2})\dots\mu(m_{l-1})\mu(t_{1})\mu(m_{l+1})\dots\mu(m_{p})}=\frac{\alpha_{2}}{\alpha_{1}}\cdot\mu_{\sigma}\cdot P_{\mu(m_{1})\mu(m_{2})\dots\mu(m_{l-1})\mu(t_{2})\mu(m_{l+1})\dots\mu(m_{p})}
    \end{equation*}
    So it follows that:
    \begin{equation*}
        \mu(\sigma(m_{1},m_{2},\dots,m_{l-1},t_{1},m_{l+1},\dots,m_{p}))=\frac{\alpha_{2}}{\alpha_{1}}\cdot\mu(\sigma(m_{1},m_{2},\dots,m_{l-1},t_{2},m_{l+1},\dots,m_{p}))
    \end{equation*}
    Now, since the depth of $\context$ in $c'$ is $h-1$, from the induction hypothesis we obtain that:
    \begin{equation*}
        H[\sigma(t_{1},t_{2},\dots,t_{l-1},t_{1},t_{l+1},\dots,t_{p})][c']=\frac{\alpha_{2}}{\alpha_{1}} H[\sigma(t_{1},t_{2},\dots,t_{l-1},t_{2},t_{l+1},\dots,t_{p})][c']
    \end{equation*}
    So:
    \begin{equation*}
        H[t_{1}][c]=\frac{\alpha_{2}}{\alpha_{1}}\cdot H[t_{2}][c]
    \end{equation*}
    As required.
\end{proof}
\begin{prop}\label{prop:finiteClasses}
    Let $H$ be the Hankel Matrix of a language generated by a CMTA, then $\equiv_{H}$ has a finite number of equivalence classes.
\end{prop}
\begin{proof}
    By Lemma \ref{lemma:oneHotVec} we have that for every tree $t$, $\mu(t)=\alpha\cdot v_{i}$ for some non-negative constant $\alpha$ and some $i$, where $v_{i}$ is the $i$'th standard basis vector. Let $t_{1},t_{2}$ be two trees s.t. $\mu(t_{1})=\alpha_{1}\cdot v_{i}\neq\bar{0}$ and $\mu(t_{2})=\alpha_{2}\cdot v_{2}\neq\bar{0}$. By Lemma \ref{lemma:contextMaintainsOneHot} we have that for every context $c$:
    \begin{equation*}
         H[t_{1}][c]=\frac{\alpha_{2}}{\alpha_{1}} H[t_{2}][c]
    \end{equation*}
    So $t_{1}\equiv_{H} t_{2}$.
    
    Since there are at most $d$ values possible for $i$, where $d$ is the dimension of the MTA, it follows that $\equiv_{H}$ has $d+1$ equivalence classes. One for each value of $i$ and another for all trees s.t. $\mu(t)=\bar{0}$.
\end{proof}

In Figure \ref{fig:cmta_equivalence_classes} the Hankel Matrix of the grammar \ref{CMTAExample} is shown, with the different equivalence classes highlighted in different colors.
\begin{figure}
    \centering
    \begin{tikzpicture}
    \node[draw=none] at (0,0) {      \begin{tabular}{ c|c|c|c|c|c|c } 
          & \begin{tikzpicture}\node[shape=circle,draw=none] (A) at (0,0) {$\context$};\end{tikzpicture} &     \begin{tikzpicture}
     \node[shape=circle,draw=none] (root) at (0.5,0.5) {\tiny{$b$}};
     \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$\context$}};
     \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$a$}};
     \path [-] (root) edge node[above] {} (A);
     \path [-] (root) edge node[above] {} (A2);
     \end{tikzpicture}  &
          \begin{tikzpicture}
     \node[shape=circle,draw=none] (root) at (0.5,0.5) {\tiny{$b$}};
     \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$a$}};
     \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$\context$}};
     \path [-] (root) edge node[above] {} (A);
     \path [-] (root) edge node[above] {} (A2);
     \end{tikzpicture} & 
     \begin{tikzpicture}
         \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
         \node[shape=circle,draw=none] (A) at (0,0.5) {\tiny{$a$}}; 
         \node[shape=circle,draw=none] (root2) at (1,0.5) {\tiny{$b$}};
         \node[shape=circle,draw=none] (A3) at (0.5,0) {\tiny{$\context$}};
         \node[shape=circle,draw=none] (A4) at (1.5,0) {\tiny{$a$}};
         \path [-] (root) edge node[above] {} (root2);
         \path [-] (root) edge node[above] {} (A);
         \path [-] (root2) edge node[above] {} (A3);
         \path [-] (root2) edge node[above] {} (A4);
     \end{tikzpicture}
     &   \begin{tikzpicture}
         \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
         \node[shape=circle,draw=none] (A) at (0,0.5) {\tiny{$a$}}; 
         \node[shape=circle,draw=none] (root2) at (1,0.5) {\tiny{$b$}};
         \node[shape=circle,draw=none] (A3) at (0.5,0) {\tiny{$a$}};
         \node[shape=circle,draw=none] (A4) at (1.5,0) {\tiny{$\context$}};
         \path [-] (root) edge node[above] {} (root2);
         \path [-] (root) edge node[above] {} (A);
         \path [-] (root2) edge node[above] {} (A3);
         \path [-] (root2) edge node[above] {} (A4);
     \end{tikzpicture}
     & $\hdots$
     \\ \hline
     \rowcolor{gray!70}
         \begin{tikzpicture}\node[shape=circle,draw=none] (A) at (0,0) {$a$};\end{tikzpicture} & $0$ & $\frac{1}{2}$ & $\frac{1}{2}$ & $0$ & $0$ & $\ddots$ \\ \hline
           \rowcolor{gray!40}
         \begin{tikzpicture}
2     \node[shape=circle,draw=none] (root) at (0.5,0.5) {\tiny{$b$}};
     \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$a$}};
     \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$a$}};
     \path [-] (root) edge node[above] {} (A);
     \path [-] (root) edge node[above] {} (A2);
     \end{tikzpicture} & $\frac{1}{2}$ & $0$ & $0$ & $\frac{1}{8}$ & $0$ & $\ddots$ \\  \hline
           \rowcolor{gray!10}
         \begin{tikzpicture}
         \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
         \node[shape=circle,draw=none] (A) at (0,0.5) {\tiny{$a$}}; 
         \node[shape=circle,draw=none] (root2) at (1,0.5) {\tiny{$b$}};
         \node[shape=circle,draw=none] (A3) at (0.5,0) {\tiny{$a$}};
         \node[shape=circle,draw=none] (A4) at (1.5,0) {\tiny{$a$}};
         \path [-] (root) edge node[above] {} (root2);
         \path [-] (root) edge node[above] {} (A);
         \path [-] (root2) edge node[above] {} (A3);
         \path [-] (root2) edge node[above] {} (A4);
     \end{tikzpicture} & $0$ & $0$ & $0$ & $0$ & $0$ & $\ddots$ \\  \hline
           \rowcolor{gray!10}
         \begin{tikzpicture}
             \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
             \node[shape=circle,draw=none] (A) at (1,0.5) {\tiny{$a$}}; 
             \node[shape=circle,draw=none] (root2) at (0,0.5) {\tiny{$b$}};
             \node[shape=circle,draw=none] (A3) at (-0.5,0) {\tiny{$a$}};
             \node[shape=circle,draw=none] (A4) at (0.5,0) {\tiny{$a$}};
             \path [-] (root) edge node[above] {} (root2);
             \path [-] (root) edge node[above] {} (A);
             \path [-] (root2) edge node[above] {} (A3);
             \path [-] (root2) edge node[above] {} (A4);
         \end{tikzpicture}
         & $0$ & $0$ & $0$ & $0$ & $0$ & $\ddots$ \\  \hline
            \rowcolor{gray!40}
         \begin{tikzpicture}
         \node[shape=circle,draw=none] (root) at (-0.25,1) {\tiny{$b$}};
         \node[shape=circle,draw=none] (root2) at (-0.75,0.5) {\tiny{$b$}}; 
         \node[shape=circle,draw=none] (root3) at (0.25,0.5) {\tiny{$b$}};
         \node[shape=circle,draw=none] (A1) at (-1,-0.25) {\tiny{$a$}};
         \node[shape=circle,draw=none] (A2) at (-0.5,-0.25) {\tiny{$a$}};
         \node[shape=circle,draw=none] (A3) at (0,-0.25) {\tiny{$a$}};
         \node[shape=circle,draw=none] (A4) at (0.5,-0.25) {\tiny{$a$}};
         \path [-] (root) edge node[above] {} (root2);
         \path [-] (root) edge node[above] {} (root3);
         \path [-] (root2) edge node[above] {} (A1);
         \path [-] (root2) edge node[above] {} (A2);
         \path [-] (root3) edge node[above] {} (A3);
         \path [-] (root3) edge node[above] {} (A4);
     \end{tikzpicture}
     & $\frac{1}{8}$ & $0$ & $0$ & $\frac{1}{32}$ & $0$ & $\ddots$ \\  \hline
         $\vdots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$
        \end{tabular}};
    \end{tikzpicture}
    \caption{The Hankel Matrix of the grammar \ref{CMTAExample}. The different equivalence classes are highlighted with different shades. Note that $b(a,a)\treesColin{4}{H} b(b(a,a),b(a,a))$.}
    \label{fig:cmta_equivalence_classes}
\end{figure}
\subsubsection{Relating CMTA and SUWCFG}
\begin{prop}\label{prop:colinearity}
Let $H$ be the Hankel Matrix of an SUWCFG. 
	Let $t_{1},t_{2}$ be derivation trees rooted by the same non-terminal $N_i$. Assume $\Prob(t_{1}),\Prob(t_{2})>0$.
	Then $t_{1}\treesColin{\alpha}{H} t_{2}$ for some $\alpha\neq 0$.
\end{prop}

\begin{proof}
	Let $c$ be a context. Let $u\context v$ be the  yield of the context; that is, the letters with which the leaves of the context are tagged, in a left to right order. Note that $u$ and $v$ might be $\varepsilon$. 
	We denote by $\Prob_{i}(c)$ the probability of deriving this context, while setting the context location to be $N_{i}$. That is:
	\begin{equation*}
	\Prob_{i}(c)=\Prob(S\underset{\mathcal{G}}{\overset{*}{\rightarrow}} u N_{i} v)
	\end{equation*}
	Let $\Prob(t_{1})$ and $\Prob(t_{2})$ be the probabilities for deriving the trees $t_{1}$ and $t_{2}$ respectively. So we obtain:
	
	\begin{align*}
	\Prob(\contextConcat{c}{t_{1}})&=\Prob_{i}(c)\cdot \Prob(t_{1})\\
	\Prob(\contextConcat{c}{t_{2}})&=\Prob_{i}(c)\cdot \Prob(t_{2})
	\end{align*}
	So we obtain, for every context $c$, assuming that $P_{i}(c)\neq 0$:
	\begin{equation*}
	\frac{\Prob(\contextConcat{c}{t_{1}})}{\Prob(\contextConcat{c}{t_{2}})}=\frac{\Prob(t_{1})}{\Prob(t_{2})}
	\end{equation*}
	For a context $c$ s.t. $P_{i}(c)=0$ we obtain that $\Prob(\contextConcat{c}{t_{1}})=\Prob(\contextConcat{c}{t_{2}})=0$. So for every context:
	\begin{equation*}
	\Prob(\contextConcat{c}{t_{1}})=\frac{\Prob(t_{1})}{\Prob(t_{2})}\Prob(\contextConcat{c}{t_{2}})
	\end{equation*}
	So $H[t_{1}]=\alpha\cdot H[t_{2}]$ for $\alpha=\frac{\Prob(t_{1})}{\Prob(t_{2})}$, so $H[t_{1}]$ and $H[t_{2}]$ are co-linear, and $t_{1}\treesColin{\alpha}{H} t_{2}$.
\end{proof}

\begin{cor}\label{cor:finite-equiv-cls}
The skeletal tree-set for an SUPCFG has a finite number of equivalence classes under $\equiv_{H}$.
\end{cor}
\begin{proof}
	Since the PCFG is structurally unambiguous, it follows that for every skeletal tree $s$ there is a single tagged parse tree $t$ s.t. $\skel(t)=s$. So for every $s$ there is a single possible tagging, and a single possible non-terminal in the root. By Proposition \ref{prop:colinearity} every two trees $s_{1},s_{2}$  which are tagged by the same non-terminal, and in which $\Prob(s_{1}),\Prob(s_{2})>0$ are in the same equivalence class under $\equiv_{H}$. There is another equivalence class for all the trees $t\in\trees$ s.t. $\Prob(t)=0$. Since there is a finite number of non-terminals, there is a finite number of equivalence classes under $\equiv_{H}$.
\end{proof}

\newcommand{\DerivationRhs}{x}

To show that the resulting PMTA is a CMTA we
need the following lemma.
We recall that a CFG $\grmr{G}=\langle \Vars,\Sigma,R,S\rangle$ is said to be
invertible if and only if $A \rightarrow \DerivationRhs$ and $B \rightarrow \DerivationRhs$, for $\DerivationRhs\in(\Vars\cup\Sigma)^{*}$ in $R$ implies $A = B$.

\begin{lem}\label{lem:invertible-iff-structuambig}
A CFG is invertible iff it is structurally unambiguous
\end{lem}
\begin{proof}
Let $\grmr{G}$ be a SUCFG. We  show that $\grmr{G}$ is invertible. Assume towards contradiction that there are derivations $N_{1}\rightarrow\DerivationRhs$ and $N_{2}\rightarrow\DerivationRhs$. Then the tree $?(\DerivationRhs)$ is structurally ambiguous since its root can be tagged by both $N_{1}$ and $N_{2}$.

Let $\grmr{G}$ be an invertible grammar. We  show that $\grmr{G}$ is an SUCFG. Let $t$ be a skeletal tree. We show by induction on the height of $t$ that there is a single tagging for $t$.

For the base case, the height of $t$ is $1$. Therefore, $t$ is a leaf so obviously, it has a single tagging.

For the induction step, we  assume that the claim holds for all skeletal trees of height at most $h\geq 1$. Let $t$ be a tree of height $h+1$. Then $t=?(t_{1},t_{2},...,t_{p})$ for some trees $t_{1},t_{2},...,t_{p}$ of smaller depth. By the induction hypothesis, for each of the trees $t_{1},t_{2},...,t_{p}$ there is a single possible tagging. 
Hence we have established that all nodes of $t$, apart from the root, have a single tagging.
Let $X_{i}\in\Sigma\cup N$ be the only possible tagging for the root of $t_{i}$. Let $\DerivationRhs=X_{1}X_{2}...X_{p}$. Since the grammar is invertible, there is a single non-terminal $N$ s.t. $N\rightarrow\DerivationRhs$. Hence, there is a single tagging for the root of $t$ as well. Thus $\grmr{G}$ is structurally unambiguous.
\end{proof}

We are finally ready to prove the following proposition:
\begin{prop}\label{prop:SUWCFGhaveCMTA}
    A CMTA can represent an SUWCFG.
\end{prop}
\begin{proof}
    By Proposition~\ref{prop:equiv2} a WCFG $\tuple{\grmr{G},\theta}$ %, which is a special case of WCFG, 
    can be represented by a PMTA $\aut{A}_{\grmr{G}}$, namely they provide the same weight for every
    skeletal tree. By Lemma~\ref{lem:invertible-iff-structuambig} the fact that $\grmr{G}$ is unambiguous implies
    it is invertible. We show that given $\grmr{G}$ is invertible, the 
    resulting PMTA is actually a CMTA. That is, in every column of the matrices of $\aut{A}_{\grmr{G}}$,
    there is at most one non-zero coefficient. Let $\alpha\in (\Sigma\cup \Vars)^{p}$, let $\iota(\alpha)$ be the extension of $\iota$ to $\alpha$ (e.g. $\iota(aN_7bb)=\iota(a)\iota(N_7)\iota(b)\iota(b)$).
    Since $\grmr{G}$ is invertible, there is a single $N_{i}$ from which $\alpha$ can be derived, namely for which
     $\grmrwgt{N_{i}}{t^{N_i}_\alpha}>0$ where $t^{N_i}_\alpha$ is a tree deriving $\alpha$ with $N_i$ in the root.
     If $\alpha\in\Sigma$, i.e. it is a leaf, then we have that $\mu_\sigma[j]=0$ for every $j\neq i$, and $\mu_\sigma[i]>0$. If $\alpha\notin\Sigma$, then we have that ${{\mu_?}^{j}}_{\iota(\alpha)}=0$ for every $j\neq i$, and ${{\mu_?}^{i}}_{\iota(\alpha)}>0$, as required.
\end{proof}
\subsubsection{Learning CMTA}\label{sec:cstar}
We are now ready to present our learning algorithm for Co-linear Multiplicity Tree Automata. We term this algoritm \cstar. Using this algorithm, and following what we've shown in Proposition \ref{prop:SUWCFGhaveCMTA}, we can use \cstar\ to learn SUWCFGs, those can later be converted, following \cite{abney1999relating, smith2007weighted} to SUPCFGS. Figure \ref{fig:learning_diagram} portrays our learning scheme, from an oracle which can answer structured membership and equivalence queries to an SUPCFG.
\begin{figure}
    \centering
    \begin{tikzpicture}
        \node[shape=rectangle,draw=black,rounded corners,] (A1) at (0,0) {Oracle};
    	\node[shape=rectangle,draw=black,rounded corners,] (A2) at (2.5,0) {CMTA};
    	\node[shape=rectangle,draw=black,rounded corners,] (A3) at (6,0) {SUWCFG};
    	\node[shape=rectangle,draw=black,rounded corners,] (A4) at (11,0) {SUPCFG};
    	\path[->,draw,thick] (A1) edge node[above] {\cstar} (A2);
    	\path[->,draw,thick] (A2) edge node[above, align=center] {Proposition\\ \ref{prop:equiv1}} (A3);
    	\path[->,draw,thick] (A3) edge node[above, align=center] {\cite{abney1999relating, smith2007weighted}} (A4);
    \end{tikzpicture}
    \caption{Our learning scheme. Using an oracle which can answer structured membership and equivalence queries on some unknown SUPCFG $\mathcal{G}$ to learn the unknown grammar.}
    \label{fig:learning_diagram}
\end{figure}

Our algorithm, which is given in Alg~\AlgLearnCMTA, is a variation of the \lstar\ algorithm. We maintain an observation table, a sub-matrix of the infinite Hankel Matrix, which we fill using membership queries, and try to make it closed (Alg~\AlgCloseCMTA) and consistent (Alg~\AlgConsistentCMTA). (The definitions of closed and consistent with regards to our algorithm will follow shortly.) After the table is closed and consistent, we extract a CMTA from it (Alg~\AlgExtractCMTA), and ask an equivalence query. If the answer is positive we halt, and return the CMTA, otherwise we add all prefixes of the counter example to the rows of the table and continue.

The algorithm maintains two sets, $T\subseteq \trees(\Sigma)$ and $C\subseteq\trees_{\context}(\Sigma)$ s.t. both $T$ and $C$ are prefix-closed. We define $H(T,C)$ to be the sub-matrix of $H$, the infinite Hankel Matrix, restricted to the rows of $T$ and columns of $C$, this is our observation table.
We will now define a \emph{closed} and \emph{consistent} observation table. To do that, we first need the following definition:

\begin{defi}
Given a set of trees $T$ and a ranked alphabet $\Sigma$, we use $\Sigma(T)$ for the set of trees:
\begin{equation*}
	\Sigma(T)=\{\sigma(t_{1},t_{2},\hdots,t_{k}):\exists \Sigma_{k}\in\Sigma,\sigma\in\Sigma_{k},t_{i}\in T, 1\leq i\leq k\}
\end{equation*}
\end{defi}

For example, if $\Sigma=\{\Sigma_{0}=\{a,b\},\Sigma_{2}=\{?\}\}$ and  $T=\{a,b \}$ then:
\begin{equation*}
	\Sigma(T)=\{?(a,a),?(a,b),?(b,a),?(b,b)\}
\end{equation*}

An observation table $H(T,C)$ is termed \emph{closed} if for every $t\in\Sigma(T)$ s.t. $H[T]\neq 0$:
\begin{equation*}
	t\treesColin{\alpha}{H[T][C]} t'
\end{equation*}
for some $t'\in T,\alpha>0$.

Algorithm \AlgCloseCMTA makes an observation table closed.

Now, we define a \emph{consistent} observation table. First we need the following definitions:
\begin{defi}
We use $\Sigma(T,t)$ for the set of trees in $\Sigma(T)$ satisfying that one of the children is the tree $t$.
\end{defi}
For example, for $T=\{a,?(a,a)\}$ and $t=\{a\}$ we have that
\begin{equation*}
    \Sigma(T,t)=\{?(a,a),?(a,?(a,a)),?(?(a,a),a)\}
\end{equation*}


\begin{defi}
We use $\Sigma(T,\context)$ for the set of contexts all of whose children are in $T$. 
\end{defi}

For example, for $T=\{a,?(a,a)\}$ 

\begin{equation*}
    \Sigma(T,\context)=\{?(\context,a),?(\context,?(a,a)),?(a,\context), ?(?(a,a),\context)\}
\end{equation*}

\begin{defi}
An observation table $H(T,C)$ is said to be \emph{zero-consistent} if for every $t\in T$ s.t. $H(T,C)[t]=0$ we have that:
\begin{equation*}
	H(T,C)[t']=0
\end{equation*}
For every $t'\in\Sigma(T,t)$.
\end{defi}
If a table isn't zero-consistent, that is -- there exists a tree $t$ s.t. $H[t]=\bar{0}$ but there exists $t'\in\Sigma(T,t)$ s.t. $H[t']\neq\bar{0}$ then we add the context $c\in\Sigma(T,\context)$ s.t. $t'=\contextConcat{c}{t}$ to $C$. This is what the first loop of Alg.~\AlgConsistentCMTA does. Figure \ref{fig:zero_consistent} shows how a context is added to a non-zero-consistent observation table to make it zero-consistent.
%\definecolor{addedColumn}{rgb}{0.2,0.8,1.0}
\definecolor{addedColumn}{rgb}{.95,.95,.96}
\begin{figure}
    \centering
    \begin{tabular}{ c|c|c } 
      & $\context$  &  \cellcolor{addedColumn}$?(\context,a)$  \\ \hline
     $a$ & $0$ & \cellcolor{addedColumn}$\frac{1}{2}$ \\ \hline
     $?(a,a)$ & $\frac{1}{2}$ &  \cellcolor{addedColumn}$0$  \\  \hline
     $\boldsymbol{?(a,b(a,a))}$ & $0$ & \cellcolor{addedColumn}$0$ \\  \hline
     $\boldsymbol{?(b(a,a),a)}$ & $0$ & \cellcolor{addedColumn}$0$   \\  \hline
     $\boldsymbol{?(?(a,a),?(a,a))}$ & $\frac{1}{8}$ & \cellcolor{addedColumn}$0$  \\  
    \end{tabular}
    \caption{An observation table, with $T=\{a,?(a,a)\}$ and $C=\{\context\}$. The table isn't zero-consistent, since $H(T,C)[a]=\bar{0}$ but for $?(a,a)\in\Sigma(T,a)$ we have that $H(T,C)[?(a,a)]\neq\bar{0}$. This problem is solved by adding the context $?(\context,a)$ (the grayed context) to $C$.}
    \label{fig:zero_consistent}
\end{figure}
\begin{defi}
An observation table $H(T,C)$ is said to be \emph{co-linear-consistent} if for every $t_{1},t_{2}\in T$ s.t. $t_{1}\treesColin{\alpha}{H[T][C]} t_{2}$, and every $c\in\Sigma(T,\context)$
\begin{equation*}
	\contextConcat{c}{t_{1}}\treesColin{\alpha}{H[T][C]}\contextConcat{c}{t_{2}}
\end{equation*}
\end{defi}

\begin{defi}
An observation table is consistent if it is both zero consistent and co-linear consistent.
\end{defi}
\begin{algorithm}[H]\label{alg:cstarClose}
\caption{$C^{*}$ close}
\begin{algorithmic}[1]
\Procedure{close}{$T,C,H,B$}
\While {$\exists t\in\Sigma(t)$ s.t. $H[t]$ is co-linearly independent from $t$}
\State $B\gets B\cup\{t\}$
\State $T\gets B\cup\{t\}$
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]\label{alg:cstarConsistent}
\caption{$C^{*}$ consistent}
\begin{algorithmic}[1]
\Procedure{consistent}{$T,C,H,B$}
\For {$t\in T$ s.t. $H[t]=\bar{0}$}
\For {$c\in\Sigma(t,\context),c'\in C$} \Comment{Checks zero-consistency}
\If {$\mq(\contextConcat{c'}{\contextConcat{c}{t}})\neq 0$}
\State $C\gets C\cup\{\contextConcat{c}{c'}\}$
\EndIf
\EndFor
\EndFor
\For {$t_{1},t_{2}\in T$ s.t. $t_{1}\treesColin{\alpha}{H(T,C)} t_{2}$} \Comment{Checks co-linear-consistency}
\For {$c\in\Sigma(T,\context),c'\in C$}
\If {$H[c'][\contextConcat{c}{t_{1}}]\neq\alpha\cdot H[c'][\contextConcat{c}{t_{2}}]$}
\State $C\gets C\cup\{\contextConcat{c}{c'}\}$
\EndIf
\EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]\label{alg:cstarComplete}
\caption{$C^{*}$ complete}
\begin{algorithmic}[1]
\Procedure{complete}{$T,C,H,B,S$}
\State $T\gets T\cup S$
\While {$(T,C,H,B)$ is not closed or not consistent}
\State $\textsc{close}(T,C,H,B)$
\State $\textsc{consistent}(T,C,H,B)$
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]\label{alg:cstarExtract}
\caption{Extract CMTA}
\begin{algorithmic}[1]
\Procedure{extract\_cmta}{$T,C,H,B$}
\State $d\gets |B|$
\For {$0\leq k\leq p$}
\For {$\sigma\in \Sigma_{(k)}$}
\For {$(i_{1},i_{2},\dots,i_{k})\in \{1,2,\dots,d\}^{k}$}
\State Let $t=\sigma(b_{i_{1}},b_{i_{2}},\dots,b_{i_{k}})$
\If {$H[t]=\bar{0}$}
\For {$1\leq j\leq d$}
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets 0$
\EndFor
\Else
\State Let $b_{i}\in B,\alpha\in\mathbb{R}$ be s.t. $t_{i_{1},i_{2},\dots,i_{k}}\treesColin{\alpha}{H} b_{i}$
\For {$1\leq j\leq d$}
\If {$j=i$}
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets\alpha$
\Else
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets 0$
\EndIf
\EndFor
\State Let $\mu_{\sigma}$ be the $d\times d^{k}$ matrix obtained from the respective coefficients.
\EndIf
\EndFor
\EndFor
\EndFor
\For {$1\leq j\leq d$}
\State $\lambda[i]\gets H(\context,b_{i})$
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[H]\label{alg:cstarLearn}
\caption{$C^{*}$}
\begin{algorithmic}[1]
\Procedure{learn}{}
\State Initialize $B\gets \emptyset,T\gets\emptyset,C\gets\{\context\}$
\State $\textsc{complete}(T,C,H,B,\Sigma_{0})$
\While {true}
\State $\mathcal{A}\gets$ \textsc{extract\_cmta}(T,C,H,B)
\State $t\gets\seq(\mathcal{A})$
\If {$t=\textsl{null}$}
\State return $\mathcal{A}$
\Else
\State $\textsc{complete}(T,C,H,B,\textsl{pref}(t))$
\EndIf
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}
To prove the main theorem we require a series of lemmas, which we state and prove here.

We start with some additional notations.
Let $v$ be a row vector in a given matrix. Let $C$ be a set of columns. We denote by $v[C]$ the restriction of $v$ to the columns of $C$. For a set of row-vectors $V$ in the given matrix, we denote by $V[C]$ the restriction of all vectors in $V$ to the columns of $C$.


\begin{lem}\label{lemmaContextColin}
	Let $B$ be a set of vectors in a matrix $H$, and let $C$ be a set of columns. If a row $v[C]$ is co-linearly independent from $B[C]$ then $v$ is co-linearly independent from $B$.
\end{lem}
\begin{proof}
	Assume towards contradiction that there is a vector $b\in B$ and a scalar $\alpha\in\reals$ s.t. $v=\alpha b$. Then for every column $c$ we have $v[c]=\alpha b[c]$. In particular that holds for every $c\in C$. Thus, $v[C]=\alpha b[C]$ and so $v[C]$ is not co-linearly independent from $B[C]$, contradicting our assumption.
\end{proof}



\begin{lem}\label{replacementLemma}
	Let $\aut{A}=(\Sigma,\mathbb{R},d,\mu,\lambda)$ %(\mu,\lambda,V)$ 
	be a CMTA. Let $t_{1},t_{2}$ s.t. $\mu(t_{1})=\alpha\cdot\mu(t_{2})$. Then for every context $c$:
	\begin{equation*}
	\mu(\contextConcat{c}{t_{1}})=\alpha\cdot\mu(\contextConcat{c}{t_{2}})
	\end{equation*}
\end{lem}	
	\begin{proof}
		The proof is by induction on the depth of $\context$ in $c$.
		
	For the base case, 	the depth of $\context$ in $c$ is $1$. Hence, $c=\context$ and indeed we have:
			\begin{equation*}
			\mu(\contextConcat{c}{t_{1}})=\mu(t_{1})=\alpha\cdot\mu(t_{2})=\alpha\cdot\mu(\contextConcat{c}{t_{2}})
			\end{equation*}
			As required.
		 
		
		For the induction step, 
		 assume the claim holds for all contexts where $\context$ is in depth at most $h$. Let $c$ be a context s.t. $\context$ is in depth $h+1$. Hence, there exists contexts $c_1$ and $c_2$ s.t.  $c=\contextConcat{c_{1}}{c_{2}}$ where $c_{2}=\sigma(s_{1},s_{2},...,s_{i-1},\context,s_{i+1},...,s_{p})$ for some $s_i$'s and the depth of $\context$ in $c_{1}$ is $h$. Let $t'_{1}=\contextConcat{c_{2}}{t_{1}}$ and let $t'_{2}=\contextConcat{c_{2}}{t_{2}}$ We have:
		 {\small{
		\begin{align*}
		\mu(t'_{1})&=
		\mu(\contextConcat{c_{2}}{t_{1}})\\
		&=\mu_{\sigma}(\mu(s_{1}),\mu(s_{2}),...,\mu(s_{i-1}),\mu(t_{1}),\mu(s_{i+1}),...,\mu(s_{p}))\\
		&=\mu_{\sigma}(\mu(s_{1}),\mu(s_{2}),...,\mu(s_{i-1}),\alpha\cdot\mu(t_{2}),\mu(s_{i+1}),...,\mu(s_{p}))
		\end{align*}}}
		Similarly for $t_{2}$ we obtain:
		\begin{equation*}
		\mu(t'_{2})=\mu_{\sigma}(\mu(s_{1}),\mu(s_{2}),...,\mu(s_{i-1}),\mu(t_{2}),\mu(s_{i+1}),...,\mu(s_{p}))\\
		\end{equation*}
		By properties of multi-linear functions we obtain:
		\begin{equation*}
		\begin{array}{rl}
		\mu(\sigma(s_{1},s_{2},...,s_{i-1},t_{1},s_{i+1},...,s_{p}))&=\\
		\alpha\cdot\mu(\sigma(s_{1},s_{2},...,s_{i-1},t_{2},s_{i+1},...,s_{p}))
		\end{array}
		\end{equation*}
		
		
		
		Thus, $\mu(t'_{1})=\alpha\cdot\mu(t'_{2})$, and by the induction hypothesis on $c_{1}$ we have:
		\begin{equation*}
		\mu(\contextConcat{c_{1}}{t'_{1}})=\alpha\cdot\mu(\contextConcat{c_{1}}{t'_{2}})
		\end{equation*}
		So:
		\begin{equation*}
		\mu(\contextConcat{c}{t_{1}})=\mu(\contextConcat{c_{1}}{t'_{1}})=\alpha\cdot\mu(\contextConcat{c_{1}}{t'_{2}})=\alpha\cdot\mu(\contextConcat{c}{t_{2}})
		\end{equation*}
		As required.	
\end{proof}

A subset $B$ of $T$ is called a \emph{basis} if for every ${t\in T}$, if ${H[t]\neq 0}$ then there is a unique $b\in B$, s.t. $t\treesColin{\alpha}{H} b$.
%
Let $(T,C,H,B)$ be an observation table. Then $B=\{b_1,b_2\ldots,b_d\}$ is a {basis} for $T$, and if $b_i$ is the unique element of $B$ s.t. $t\treesColin{\alpha}{H} b_i$,
we say that $\classrepr{t}{B}=b_{i}$, $\classcoeff{t}{B}=\alpha$, and $\classind{t}{B}=i$. 

The following lemma states that the value assigned to a tree $?(t_{1},t_{2},...,t_{p})$ all of whose children are in $T$, 
can be computed by multiplying the respective coefficients $\classcoeff{t_i}{B}$ witnessing the co-linearity of $t_i$ to its respective
base vector $\classrepr{t_i}{B}$.

\begin{lem}\label{consistencyExpansion}
	Let $(T,C,H,B)$  be a closed consistent observation table. Let $t_{1},t_{2},...,t_{p}\in T$, and let $t=?(t_{1},t_{2},...,t_{p})$. Then:
	\begin{equation*}
	H[?(t_{1},t_{2},...,t_{p})]=\prod_{i=1}^{p}\classcoeff{t_{i}}{B}\cdot H[?(\classrepr{t_{1}}{B},\classrepr{t_{2}}{B},...,\classrepr{t_{p}}{B})]
	\end{equation*}
\end{lem}	
	

	\begin{proof}
		Let $k$ be the number of elements in $t_{1},t_{2},...,t_{p}$  s.t. $t_{i}\neq\classrepr{t_{i}}{B}$. We proceed by induction on $k$. 
		
		For the base case, we have $k=0$, so for every $t_{i}$ we have $t_{i}=\classrepr{t_{i}}{B}$ and $\classcoeff{t_{i}}=1$. Hence, obviously we have:
		\begin{equation*}
		H[?(t_{1},t_{2},...,t_{p})]=\prod_{i=1}^{p}\classcoeff{t_{i}}{B}\cdot H[?(\classrepr{t_{1}}{B},\classrepr{t_{2}}{B},...,\classrepr{t_{p}}{B})]
		\end{equation*}
		
		Assume now the claim holds for some ${k\geq 0}$. Since ${k+1>0}$ there is at least one $i$  s.t. $t_{i}\neq\classrepr{t_{i}}{B}$. Let $t'=?(t_{1},t_{2},...,t_{i-1},\classrepr{t_{i}}{B},t_{i+1},...,t_{p})$. Since the table is consistent, we have that $H[t]=\classcoeff{t_{i}}{B}\cdot H[t']$.
		Now,  $t'$ has $k$ children  s.t. $t_{i}\neq\classrepr{t_{i}}{B}$, so from the induction hypothesis we have:
		\begin{equation*}
		H[t']=\prod_{\begin{array}{c}{j=1}\\{j\neq i}\end{array}}^{p}\classcoeff{t_{j}}{B}\cdot H[?(\classrepr{t_{1}}{B},\classrepr{t_{2}}{B},...,\classrepr{t_{p}}{B})
		\end{equation*}
		So we have:
		\begin{equation*}
		H[t]=\classcoeff{t_{i}}{B}\cdot H[t']=\prod_{j=1}^{p}\classcoeff{t_{j}}{B}\cdot H[?(\classrepr{t_{1}}{B},\classrepr{t_{2}}{B},...,\classrepr{t_{p}}{B})
		\end{equation*}
		As required.
	\end{proof}


The following lemma states that if $t=?(t_{1},t_{2},...,t_{p})$  is co-linear to $s=?(s_{1},s_{2},...,s_{p})$ 
and $t_i$ is co-linear to $s_i$, for every $1\leq i\leq p$ and $H[y]\neq 0$ then the ratio between the tree coeficcient and the product of its children coefficeints is the same.
\begin{lem}\label{lem:equal-prods-coef}
		Let $t=?(t_{1},t_{2},...,t_{p})$ and $s=?(s_{1},s_{2},...,s_{p})$ s.t. $t_{i}\treesEquiv{H} s_{i}$ for $1\leq i\leq p$. 
		Then $$\frac{\classcoeff{t}{B}}{\prod_{i=1}^{p}\classcoeff{t_{i}}{B}}=\frac{\classcoeff{s}{B}}{\prod_{i=1}^{p}\classcoeff{s_{i}}{B}}$$
\end{lem}

\begin{proof}
 Let $t'=?(\classrepr{t_{1}}{B},\classrepr{t_{2}}{B} ...,\classrepr{t_{p}}{B})$.
 Note that we also have $t'=?(\classrepr{s_{1}}{B},\classrepr{s_{2}}{B},...,\classrepr{s_{p}}{B})$.
  Then from Lemma \ref{consistencyExpansion} we have that $H[t]=\prod_{i=1}^{p}\classcoeff{t_{i}}{B}\cdot H[t']$. 
  Similarly we have that $H[s]=\prod_{i=1}^{p}\classcoeff{s_{i}}{B}\cdot H[t']$. 
  Let $b=\classrepr{t}{B}=\classrepr{s}{B}$ we have $H[t]=\classcoeff{t}{B}\cdot H[b]$, and $H[s]=\classcoeff{s}{B}\cdot H[b]$.
Thus we have
\begin{equation*}
\classcoeff{t}{B}\cdot H[b]=\prod_{i=1}^{p}\classcoeff{t_{i}}{B}\cdot H[t']
\end{equation*}
And
\begin{equation*}
\classcoeff{s}{B}\cdot H[b]=\prod_{i=1}^{p}\classcoeff{s_{i}}{B}\cdot H[t']
\end{equation*}
Hence we have
\begin{equation*}
\frac{\classcoeff{t}{B}}{\prod_{i=1}^{p}\classcoeff{t_{i}}{B}}\cdot H[b]=H[t']=\frac{\classcoeff{s}{B}}{\prod_{i=1}^{p}\classcoeff{s_{i}}{B}}\cdot H[b]
\end{equation*}
Since $H[t]\neq 0$, and $t\treesEquiv{H} b\treesEquiv{H} t'$ we obtain that $H[b]\neq 0$ and $H[t']\neq 0$. 
Therefore
\begin{equation*}
\frac{\classcoeff{t}{B}}{\prod_{i=1}^{p}\classcoeff{t_{i}}{B}}=\frac{\classcoeff{s}{B}}{\prod_{i=1}^{p}\classcoeff{s_{i}}{B}}
\end{equation*}
\end{proof}

The next lemma relates the value $\mu(t)$ to  $t$'s coefficient, $\classcoeff{t}{B}$, and the vector for respective row in the basis, $\classind{t}{B}$.

\begin{lem}\label{lem:mu-t-rel}
	Let $t\in T$. If $H[t]\neq 0$ then $\mu(t)=\classcoeff{t}{B}\cdot e_{\classind{t}{B}}$. If $H[t]=0$ then $\mu(t)=0$.
\end{lem}
\begin{proof}
	The proof is by induction on the height of $t$.
	
	For the base case, $t=\sigma$ is a leaf, for some $\sigma\in\Sigma$. If $H[t]\neq 0$, by Alg.~\AlgExtractCMTA, 
	we set $\sigma^{\classind{t}{B}}$ to be $\classcoeff{t}{B}$, and for every $j\neq\classind{t}{B}$ we set $\sigma^{j}$ to be $0$, 
	so $\mu(t)=\mu_{\sigma} =\classcoeff{t}{B}\cdot e_{\classind{t}{B}}$ as required. 
	Otherwise, if $H[t]=0$ then we set $\sigma^{i}$ to be $0$ for every $i$, so $\mu(t)=0$ as required.

	
	For the induction step,  $t$ is not a leaf. Then $t=?(t_{1},t_{2},...,t_{p})$. 
	If $H[t]\neq 0$, then since $H$ is zero-consistent, we have for every $1\leq i\leq p$ that 
	$H[t_{i}]\neq 0$. So for every $1\leq j\leq p$ by induction hypothesis we have 
	$\mu(t_{j})=\classcoeff{t_{j}}{B}\cdot e_{\classind{t_{j}}{B}}$. So:
	\begin{equation*}
	\begin{array}{rl}
	\mu(t)=&\mu_{?}(\mu(t_{1}),~\ldots~,\mu(t_{p}))=\\
	=&\mu_{?}(\classcoeff{t_{1}}{B}\cdot e_{\classind{t_{1}}{B}},~\ldots~,\classcoeff{t_{p}}{B}\cdot e_{\classind{t_{p}}{B}}) \\
	\end{array}
	\end{equation*}
	

	Therefore we have:
	\begin{equation*}
	\mu(t)[j]=\sum_{j_{1},...,j_{p}\in [n]^{p}}\sigma^{j}_{j_{1},...,j_{p}}\cdot\classcoeff{t_{1}}{B} e_{\classind{t_{1}}{B}}[j_{1}]\cdots\classcoeff{t_{p}}{B} e_{\classind{t_{p}}{B}}[j_{p}]
	\end{equation*}
	

	
	Note that for every $j_{1},j_{2},...,j_{p}\neq \classind{t_{1}}{B},\classind{t_{2}}{B},...,\classind{t_{p}}{B}$ we have $\classcoeff{t_{1}}{B}\cdot e_{\classind{t_{1}}{B}}[j_{1}]~\cdots~\classcoeff{t_{p}}{B}\cdot e_{\classind{t_{p}}{B}}[j_{p}]=0$, thus
	\begin{align*}
	\mu(t)[j]&=\sigma^{j}_{\classind{t_{1}}{B},...,\classind{t_{p}}{B}}\cdot~ \classcoeff{t_{1}}{B}\cdot e_{\classind{t_{1}}{B}}[\classind{t_{1}}{B}]~\cdots~\classcoeff{t_{p}}{B}\cdot e_{\classind{t_{p}}{B}}[\classind{t_{p}}{B}]\\
	&=\sigma^{j}_{\classind{t_{1}}{B},...,\classind{t_{p}}{B}}\cdot \classcoeff{t_{1}}{B}\cdot \classcoeff{t_{2}}{B}~\cdots~\classcoeff{t_{p}}{B}
	\end{align*}
	
			
	
	By Alg.~\AlgExtractCMTA, and Lemma~\ref{lem:equal-prods-coef} we have that 	
	$$\sigma^{j}_{\classind{t_{1}}{B},\classind{t_{2}}{B},...,\classind{t_{p}}{B}}=
	\left\{ \begin{array}{l@{\quad }l} 
	0 & \mbox{if } j\neq \classind{t}{B} \\
	\frac{\classcoeff{t}{B}}{\prod_{j=1}^{p}{B}\classcoeff{t_{p}}{B}} & \mbox{if } j=\classind{t}{B}
	\end{array}\right.$$
		hence we obtain:
	\begin{align*}
	\mu(t)[\classind{t}{B}]&=\sigma^{j}_{\classind{t_{1}}{B},\classind{t_{2}}{B},...,\classind{t_{p}}{B}}\cdot \classcoeff{t_{1}}{B}\cdot \classcoeff{t_{2}}{B}\cdots \classcoeff{t_{p}}{B} \\ &=\frac{\classcoeff{t}{B}}{\prod_{j=1}^{p}\classcoeff{t_{p}}{B}}\cdot {\prod_{j=1}^{p}\classcoeff{t_{p}}{B}}=\classcoeff{t}{B}
	\end{align*}
	Thus $\mu(t)=\classcoeff{t}{B}\cdot e_{\classind{t}{B}}$ as required.
	
	If $H[t]=0$ then $\sigma^{i}_{\classind{t_{1}}{B},\classind{t_{2}}{B},...,\classind{t_{p}}{B}}=0$ for every $i$, and we obtain
	\begin{equation*}
	\mu(t)=0  
	\end{equation*}
	as required.
\end{proof}

Next we show that  rows in the basis get a standard basis vector. 

\begin{lem}\label{lemmaBase}
	For every $b_{i}\in B$, $\mu(b_{i})=e_{i}$ where $e_{i}$ is the $i$'th standard basis vector.
\end{lem}
\begin{proof}
	By induction on the height of $b_{i}$.
	
	\textbf{Base case:} $b_{i}$ is a leaf, so $b=\sigma$ for $\sigma\in\Sigma_0$. By  Alg.~\AlgExtractCMTA we set $\sigma_{i}$ to be $1$ and $\sigma_{j}$ to be $0$ for every $j\neq i$, so $\mu(b_{i})=e_{i}$.
	
	\textbf{Induction step:} $b_{i}$ is not a leaf. Note that by definition of the method $\Close$ (Alg.~\AlgCloseCMTA), all the children of $b_{i}$ are in $B$. So $b_{i}=\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{p}})$ for some base rows $b_{i_j}$'s. Let's calculate $\mu(b_{i})[j]$
	
	\begin{equation*}
	\mu(b_{i})[j]=\sum_{j_{1},j_{2},...,j_{p}\in [n]^{p}}\sigma^{j}_{j_{1},j_{2},...,j_{p}}\cdot\mu(b_{i_{1}})[j_{1}]\cdot\hdots\cdot\mu(b_{i_{p}})[j_{p}]
	\end{equation*}
	
	By the induction hypothesis, for every $1\leq j\leq p$ we have that $\mu(b_{i_{j}})[i_{j}]=1$, and $\mu(b_{i_{j}})[k]=0$ for $k\neq i_{j}$. So for every vector $j_{1},j_{2},...,j_{p}\neq i_{1},i_{2},...,i_{p}$ we obtain:
	
	\begin{equation*}
	\mu(b_{i_{1}})[j_{1}]\cdot\hdots\cdot\mu(b_{i_{p}})[j_{p}]=0
	\end{equation*}
	
	And for $j_{1},j_{2},...,j_{p}=i_{1},i_{2},...,i_{p}$ we obtain:
	
	\begin{equation*}
	\mu(b_{i_{1}})[j_{1}]\cdot\hdots\cdot\mu(b_{i_{p}})[j_{p}]=1
	\end{equation*}
	
	So we have:
	\begin{equation*}
	\mu(b_{i})[j]=\sigma^{i}_{i_{1},i_{2},...,i_{p}}
	\end{equation*}
	By Alg.~\AlgExtractCMTA we have that $\sigma^{i}_{i_{1},i_{2},...,i_{p}}=1$ and $\sigma^{j}_{i_{1},i_{2},...,i_{p}}=0$ for $j\neq i$, so $\mu(b_{i})[i]=1$ and $\mu(b_{i})[j]=0$ for $j\neq i$. Hence $\mu(b_{i})=e_{i}$ as required.
\end{proof}

The next lemma states 
for a tree $t=\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{p}})$ with
children in the basis, if 
if $t\treesColin{\alpha}{H}b_i$ then  
 $\mu(t)=\alpha\cdot  e_{i}$ where $e_{i}$ 
 is the $i$'th standard basis vector.

\begin{lem}\label{lemmaExtension}
	Let $t=\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{p}})$, s.t. ${b_{i_{j}}\in B}$ for ${1\leq j\leq p}$. Assume ${H[t]=\alpha\cdot H[b_{i}]}$ for some $i$. Then $\mu(t)=\alpha\cdot  e_{i}$.
	% where $e_{i}$ is the $i$'th standard basis vector.
\end{lem}
\begin{proof}
	If $t=\sigma$ is a leaf, then by definition we have $\sigma_{i}=\alpha$ and $\sigma_{j}=0$ for $j\neq i$, so $\mu(t)=\alpha\cdot e_{i}$.
	
	Otherwise, $t$ isn't a leaf. Assume $t=\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{p}})$. We thus have
	\begin{equation*}
	\mu(t)[j]=\sum_{j_{1},j_{2},...,j_{p}\in [n]^{p}}\sigma^{j}_{j_{1},j_{2},...,j_{p}}\cdot\mu(b_{i_{1}})[j_{1}]\cdot\hdots\cdot\mu(b_{i_{p}})[j_{p}]
	\end{equation*}
	By Lemma \ref{lemmaBase} we have that $\mu(b_{i_{j}})=e_{i_{j}}$ for $1\leq j\leq p$, hence using a similar technique to the one used in the proof of Lemma \ref{lemmaBase} we obtain that for every $1\leq j\leq p$:
	\begin{equation*}
	\mu(t)[j]=\sigma^{j}_{i_{1},i_{2},...,i_{p}}
	\end{equation*}
	
	By Alg.~\AlgExtractCMTA we have that $\sigma^{j}_{i_{1},i_{2},...,i_{p}}=\alpha$ for $i=j$ and $\sigma^{j}_{i_{1},i_{2},...,i_{p}}=0$ for $i\neq j$, so $\mu(t)=\alpha\cdot  e_{i}$ as required.
\end{proof}

The following lemma generalizes the previous lemma to any tree $t\in T$.

\begin{lem}\label{lem:Correctness}
	Let $H$ be a closed consistent sub-matrix of the Hankel Matrix. Then for every $t\in T$ s.t. $H[t]=\alpha\cdot H[b_{i}]$ we have $\mu(t)=\alpha\cdot e_{i}$
\end{lem}
\begin{proof}
	By induction on the height of $t$.
	For the base case $t$ is a leaf, and the claim holds by Lemma \ref{lemmaExtension}.
	
	Assume the claim holds for all trees of height at most $h$. Let $t$ be a tree of height $h$. Then $t=\sigma(t_{1},t_{2},...,t_{p})$. Since $T$ is prefix-closed, for every $1\leq j\leq p$ we have that $t_{j}\in T$. And from the induction hypothesis for every $1\leq j\leq p$ we have that $\mu(t_{j})=\alpha_{j}\cdot e_{i_{j}}$. Hence
	\begin{align*}
	\mu(t)&=\mu(\sigma(t_{1},t_{2},...,t_{p}))=\mu_{\sigma}(\mu(t_{1}),\mu(t_{2}),...,\mu(t_{p}))\\
	&=\mu_{\sigma}(\alpha_{1}\cdot e_{i_{1}},\alpha_{2}\cdot e_{i_{2}},...,\alpha_{p}\cdot e_{i_{p}})\\
	&=\prod_{j=1}^{p}\alpha_{j} \cdot \mu_{\sigma}(e_{i_{1}},e_{i_{2}},...,e_{i_{p}})
	\end{align*}
	Let $t'=\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{p}})$. From Lemma \ref{lemmaBase} we have
	\begin{align*}
	\mu(t)&=\prod_{j=1}^{p}\alpha_{j}\cdot\mu_{\sigma}(e_{i_{1}},e_{i_{2}},...,e_{i_{p}})\\
	&= \prod_{j=1}^{p}\alpha_{j}\cdot \mu(\sigma(\mu(b_{i_{1}}),\mu(b_{i_{2}}),...,\mu(b_{i_{p}})))\\
	&=\prod_{j=1}^{p}\alpha_{j}\cdot\mu(t')
	\end{align*}
	
	Since the table is consistent, we know that for each $1\leq j\leq p$ and $c\in C$:
	\begin{align*}
	H[\sigma(t_{1},t_{2},...,t_{j-1},t_{j},t_{j+1},...,t_{p})][c]=\\
	\alpha_{j}\cdot H[\sigma(t_{1},t_{2},...,t_{j-1},b_{i_{j}},t_{j+1},...,t_{p})][c]
	\end{align*}
	We can continue using consistency to obtain that
	\begin{align*}
	H[t][c]&=H[\sigma(t_{1},t_{2},...,t_{p})][c]\\
	&=\prod_{j=1}^{p}\alpha_{j}\cdot H[\sigma(b_{1},b_{2},...,,b_{p})][c]\\
	&=\prod_{j=1}^{p}\alpha_{j}\cdot H[t'][c]
	\end{align*}
	Thus $H[t]=\prod_{j=1}^{p}\alpha_{j}\cdot H[t']$. Let $\beta=\prod_{j=1}^{p}\alpha_{j}$, then $t\treesColin{\beta}{H} t'$. Let $b$ be the element in the base s.t. $t'\treesColin{\alpha}{H} b_{i}$. From Lemma \ref{lemmaExtension} we have that $\mu(t')=\alpha\cdot e_{i}$. Therefore $\mu(t)=\beta\cdot\alpha\cdot e_{i}$. 
	
	We have $\mu(t)=\beta\cdot\alpha\cdot e_{i}$ and $t\treesColin{\alpha\cdot\beta}{H} b_{i}$. Therefore the claim holds.
\end{proof}

We are now ready to show that for every tree $t\in T$ and context $c\in C$ the obtained CMTA
agrees with the observation table.

\begin{lem}
	For every $t\in T$ and for every $c\in C$ we have that $\mathcal{A}(\contextConcat{c}{t})=H[t][c]$
\end{lem}
\begin{proof}
	Let $t\in T$, s.t. $t\treesColin{\alpha}{H} b_{i}$ for some $b_{i}\in B$.
	The proof is by induction on the depth of $\context$ in $c$. 
	
	\textbf{Base case:} The depth of $c$ is $1$, so $c=\context$, and by lemma \ref{lem:Correctness} we have that $\mu(\contextConcat{c}{t})=\mu(t)=\alpha \cdot e_{i}$. Therefore $\mathcal{A}(t)=\alpha\cdot e_{i}\cdot\lambda$.  By Alg.~\AlgExtractCMTA we have that $\lambda[i]=H[b_{i}][\context]$. So $\mathcal{A}(t)=\alpha\cdot H[b_{i}][\context]=H[t][\context]$ as required. 
	
	\textbf{Induction step:} Let $c$ be a context s.t. the depth of $\context$ is $h+1$. So $c=\contextConcat{c'}{\sigma(t_{1},t_{2},...,t_{i-1},\context,t_{i},...,t_{p})}$ for some trees $t_j\in T$, and some context $c'$  of depth  $h$.  For each $1\leq j\leq p$, let $b_{i_{j}}$ be the element in the base, s.t. $t_{j}\equiv_{H} b_{i_{j}}$, with co-efficient $\alpha_{j}$. Let $b$ be the element in the base s.t. $t\equiv_{H} b$ with coefficient $\alpha$. Let $\widetilde{t}$ be the tree:
	\begin{equation*}
	\widetilde{t}=\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{k-1}},b,b_{i_{k}},...,b_{i_{p}})
	\end{equation*}
	Note that $\widetilde{t}\in \Sigma(B)$ and hence $\widetilde{t}\in T$. From the induction hypothesis, we obtain:
	\begin{equation*}
	\mathcal{A}(\contextConcat{c'}{\widetilde{t}})=H[\widetilde{t}][c']
	\end{equation*}
	Since the table is consistent, we have:
	\begin{align*}
	H[t][c]&=H[\sigma(t_{i_{1}},t_{i_{2}},...,t_{i_{k-1}},t,t_{i_{k}},...,t_{i_{p}})][c']\\
	&=\alpha\cdot\prod_{i=1}^{p}\alpha_{i}\cdot H[\widetilde{t}][c']
	\end{align*}
	Let $\beta=\alpha\cdot\prod_{i=1}^{p}\alpha_{i}$.
	By definition of $\aut{A}$ we have: 
	\begin{align*}
	\aut{A}(\contextConcat{c'}{\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{k-1}},b,b_{i_{k}},...,b_{i_{p}})})=\\
	\mu(\contextConcat{c'}{\sigma(b_{i_{1}},b_{i_{2}},...,b_{i_{k-1}},b,b_{i_{k}},...,b_{i_{p}})}))\cdot\lambda
	\end{align*}
	Since each $t_{i_{j}}$ is in $T$, from Proposition \ref{lem:Correctness} we have that ${\mu(t_{i_{j}})=\alpha_{j}\cdot b_{i_{j}}}$, and that ${\mu(t)=\alpha\cdot\mu(b)}$.\\
	Let $\hat{t}=\sigma(t_{i_{1}},t_{i_{2}},...,t_{i_{k-1}},t,t_{i_{k}},...,t_{i_{p}}))$.
	 So
	\begin{align*}
	\mu(\hat{t}) 
	&=\mu(\sigma(t_{i_{1}},t_{i_{2}},...,t_{i_{k-1}},t,t_{i_{k}},...,t_{i_{p}})))\\
	&=\mu_{\sigma}(\alpha_{1}\cdot b_{i_{1}},...,\alpha_{k-1}\cdot b_{i_{k-1}},\alpha\cdot b,\alpha_{k}\cdot b_{i_{k}},...,\alpha_{p}\cdot b_{i_{p}})\\
	&=\alpha\cdot\prod_{j=1}^{p}\alpha_{i}\cdot\mu_{\sigma}(b_{i_{1}},...,b_{i_{k-1}},b, b_{i_{k}},...,b_{i_{p}})\\
	&=\beta\cdot\mu(\widetilde{t})
	\end{align*}
	By Lemma \ref{replacementLemma} we have that $$\mu(\contextConcat{c'}{\sigma(t_{i_{1}},t_{i_{2}},...,t_{i_{k-1}},t,t_{i_{k}},...,t_{i_{p}})})=\beta\cdot\mu(\contextConcat{c'}{\widetilde{t}})$$
	Hence
	\begin{align*}
	\mathcal{A}(\contextConcat{c}{t})&=\mathcal{A}(\contextConcat{c'}{\sigma(t_{i_{1}},t_{i_{2}},...,t_{i_{k-1}},t,t_{i_{k}},...,t_{i_{p}})})\\
	&=\mu(\contextConcat{c'}{\sigma(t_{i_{1}},t_{i_{2}},...,t_{i_{k-1}},t,t_{i_{k}},...,t_{i_{p}})})\cdot\lambda\\
	&=\beta\cdot\mu(\contextConcat{c'}{\widetilde{t}})\cdot\lambda
	\end{align*}
	Note that all the children of $\widetilde{t}$ are in $B$, and so $\widetilde{t}\in T$. Hence, from the induction hypothesis we have:
	\begin{equation*}
	H[\widetilde{t}][c']=\mathcal{A}(\contextConcat{c'}{\widetilde{t}})=\mu(\contextConcat{c'}{\widetilde{t}})\cdot\lambda
	\end{equation*}
	So:
	\begin{equation*}
	\mathcal{A}(\contextConcat{c}{t})=\beta\cdot H[\widetilde{t}][c']=H[t][c]
	\end{equation*}
	As required.
\end{proof}


\begin{prop}
	In every iteration of Alg.\AlgLearnCMTA, the set $B$ maintained by the algorithm is contained in some correct solution.
\end{prop}
\begin{proof}
	We  show by induction that in each iteration, $B\subseteq B^{*}$ for some co-linear base $B^{*}$.
	
	The base case is trivial since $B=\emptyset$. Hence, clearly $B\subseteq B^{*}$ for some co-linear base $B^{*}$.
	
	For the induction step, let $B$ be the set created by the algorithm in the previous iteration. Let $t$ be the tree picked by the algorithm to be added to the basis in the current iteration. If $t\in B^{*}$ then $B\cup\{t\}\subseteq B^{*}$. Otherwise, $t\notin B^{*}$. Let $N$ be the tagging for the root of $t$. Since $t$ was picked, we have that $H[t][C]$ is co-linearly independent from $B[C]$. By Lemma \ref{lemmaContextColin} $H[t]$ is co-linearly independent from $B$, and so by Prop.~\ref{prop:colinearity} there is no tree in $B$ whose root is tagged by $N$. Since $B^{*}$ is a co-linear base, there must be a tree $t'\in B^{*} \setminus B$ whose root is tagged by $N$, by Prop.~\ref{prop:colinearity} $t$ and $t'$ are co-linear. Let $B^{*'}=B^{*}\setminus \{t'\}\cup \{t\}$. $B^{*'}$ is still a co-linear base, because $t$ and $t'$ are co-linear. So, $B\cup\{t\}\subseteq B^{*'}$ and $B^{*'}$ is a co-linear base.
\end{proof}

\begin{prop}\label{prop:rankInc}
	Let $(T,C,H,B)$ be a closed and consistent observation table. Let $t$ be a counterexample, and let $(T',C',H',B')=\Complete(T,C,H,$ $B,\pref(t))$. Then $|B'|>|B|$. 
\end{prop}
\begin{proof}
	Since $t$ was given as a counterexample, the previously extracted CMTA $\mathcal{A}=\textsl{CMTAB}(T,C,H,B)$ gave a wrong answer for it. By the method complete, $t\in T'$, hence by Lemma~\ref{lem:Correctness} we have that $\mathcal{A'}=\textsl{CMTAB}(T',C',H',B')$ agrees with $t$. Since we only add elements to the base, we have that $B\subseteq B'$. Now, clearly $B\neq B'$ since otherwise (following Alg.~\AlgExtractCMTA) we would obtain $\mathcal{A}=\mathcal{A'}$. Hence $B\subsetneq B'$ implying $|B'|>|B|$.
\end{proof}


We are now ready to prove the main theorem, which states that:
\begin{thm}\label{thm:bounds}
Let $n$ be the rank of the target-language, let $m$ be the size of the largest counterexample given by the teacher, and let $p$ be the highest rank of a symbol in $\Sigma$. Then the algorithm makes at most $n\cdot(n+m\cdot n+|\Sigma|\cdot (n+m\cdot n)^{p})$ $\mq$ and at most $n$ $\eq$.
\end{thm}


Before we provide the proof of the theorem we note that the complexity is polynomial in $n$ and $m$ and exponential in $p$.
If the grammar is in Chomsky Normal Form, then 
$p=2$ and hence the complexity is polynomial in all parameters.

\begin{cor}
For a grammar in Chomsky Normal Form, we have that $p=2$ and therefore the algorithm makes at most
\begin{equation*}
    n\cdot(n+m\cdot n+|\Sigma|\cdot (n+m\cdot n)^{2})
\end{equation*}
membership queries.
\end{cor}

\begin{proof}
By Prop~\ref{prop:rankInc} we have that the rank of the finite Hankel Matrix $H[C]$ increases by at least one after each equivalence query. Since the rank of the infinite Hankel Matrix $H$ is $n$, it follows that the learner makes at most $n$ equivalence queries.

For the set of contexts, the algorithm starts with $C=\{\context\}$. The algorithm adds new contexts following failed consistency checks. Each added context thus separates two trees in $T$ and increases the rank of $H[C]$ by $1$. Therefore,  $|C|\leq n$. 

We add an element to set of trees $T$ in two cases: if it is in $\Sigma(T)$, and it is co-linearly independent from $T$, or it is a prefix of a counterexample given to us by the teacher. 

The first case can occur at most $n$ times, since each time we add an element from $\Sigma(T)$ to $T$ we increase the rank of the table by $1$. 

Since the number of $\eq$ made by the learner is at most $n$, the learner receives at most $n$ counterexamples from the teacher. Let $m$ be the size of the largest counterexample given by the teacher. We add all its prefixes to $T$, so each counterexample adds at most $m$ elements to $T$. So we have that by the end of the algorithm, $|T|\leq n+m\cdot n$. Let $p$ be the maximal rank of symbol in $\Sigma$, then $|\Sigma(T)|\leq |\Sigma|\cdot |T|^{p}\leq|\Sigma|\cdot (n+m\cdot n)^{p}$. Hence the number of rows in the table is at most:
\begin{equation*}
    n+m\cdot n+|\Sigma|\cdot (n+m\cdot n)^{p}
\end{equation*}
Since the number of columns in the table is at most $n$,  the algorithm makes at most:
\begin{equation*}
    n\cdot(n+m\cdot n+|\Sigma|\cdot (n+m\cdot n)^{p})
\end{equation*}
membership queries. 

\end{proof}
\subsubsection{Running example}
We will now demonstrate a running example of the learning algorithm. 
For the unknown target  consider the series which gives probability $\frac{1}{2}^n$ to
strings of the form $a^nb^n$ for $n\geq 1$ and probability zero to all other strings. 
%\dolav{yes, but the important part is the grammar}\dana{Why? We are supposed to learn a probabilistic language, regardless of how the oracle represents it.} Note that this
 This series can be generated by the following SUPCFG $\grmr{G}=\langle \Vars,\{a,b\},R,S\rangle$
 with $\Vars=\{S,S_{2}\}$, and the following derivation rules:
$$\begin{array}{l@{\ \ \longrightarrow\ \ }lll}
S& aS_{2}~[\frac{1}{2}]\ \mid\ ab~[\frac{1}{2}]\\
S_{2}& Sb~~~[1]
\end{array}$$

The algorithm initializes $T=\{a,b\}$ and $C=\{\context\}$, fills in the entries of $M$ using $\smq$s, first for the rows of $T$ and then for their one letter extensions $\Sigma(T)$ (marked in blue), resulting   in the following observation table.
\begin{center}
	\begin{tabular}{ l | l}
		& \Tree [.$\context$ ] \\ \hline
		$a$& $0$\\ \hline
		$b$& $0$\\ \hline
		\color{blue} $?(a,a)$ & $0$\\\hline
		\color{blue} $?(a,b)$ & $0.5$\\\hline
		\color{blue} $?(b,a)$ & $0$\\\hline
		\color{blue} $?(b,b)$ & $0$\\\hline
	\end{tabular}
\end{center}

We can see that the table is not closed, since $?(a,b)\in\Sigma(T)$ but is not co-linearly spanned by $T$, so we add it to $T$. Also, the table is not consistent, since $a\treesColin{1}{H} b$, but $\mq(\contextConcat{\context}{?(a,b)})\neq\mq(\contextConcat{\context}{?(a,a)})$, so we add $?(a,\context)$ to $C$, and we obtain the following table.
From now on we  omit $0$ rows of $\Sigma(T)$ for brevity.
\begin{center}
	\begin{tabular}{l | l | l | l }
		& & \Tree [.$\context$ ] & $?(a,\context)$ \\ \hline
		$t_1$ & $a$ & $0$ & $0$ \\ \hline
		$t_2$ & $b$ & $0$ & $0.5$\\ \hline
		$t_3$ & $?(a,b)$ & $0.5$ &$ 0$ \\\hline
		& \color{blue} $?(?(a,b),b)$ & $0$ & $0.25$ \\
	\end{tabular}
\end{center}
The table is now closed but it is not zero-consistent, since we have $H[a]=\overline{0}$, but there exists a context with children in $T$, specifically $?(\context,b)$,
with which when $a$ is extended the result is not zero, namely $H[?(a,b)]\neq 0$. So we add this context
and we obtain the following table:

\vspace{2mm} 
\begin{center}
	\begin{tabular}{l | l | l | l | l }
		& & \Tree [.$\context$ ] & $?(a,\context)$ & $?(\context,b)$\\ \hline
		$t_1$ & $a$ & $0$ & $0$ & $0.5$ \\ \hline
		$t_2$ & $b$ & $0$ & $0.5$ & $0$ \\ \hline
		$t_3$ & $?(a,b)$ & $0.5$ & $0$ \\\hline
		$t_4\notin B$ & $?(a,a)$ & $0$ & $0$ & $0$ \\\hline
		& \color{blue} $?(?(a,b),b)$ & $0$ & $0.25$ & $0$ \\
	\end{tabular}
\end{center}
\vspace{2mm} 

Note that $t_{4}$ was added to $T$ since it wasn't spanned by $T$, but it is not a member of $B$, since $H[t_{4}]=0$. 
We can extract the following CMTA $\aut{A}_1=(\Sigma,\mathbb{R},d,\mu,\lambda)$ of dimension $d=3$ since $|B|=|\{t_{1},t_{2},t_{3}\}|=3$.

Let $\V=\R^3$.  For the letters $\sigma\in \Sigma_0=\{a,b\}$ we have that $\mu_\sigma:\V^0\rightarrow \V$, namely $\mu_a$ and $\mu_b$ are $3\times 3^0$-matrices. Specifically, following Alg.~\AlgExtractCMTA we get that $\mu_{a}=(1,0,0)$, $\mu_{b}=(0,1,0)$ as $a$ is the first element of $B$ and $b$ is the second.
For ${?}\in\Sigma^2$ we have that $\mu_{?}:\V^2\rightarrow \V$, thus $\mu_{?}$ is a $3\times 3^2$-matrix.
We compute the entries of $\mu_{?}$ following Alg.~\AlgExtractCMTA. For this, we consider all pairs of indices $(j,k)\in\{1,2,3\}^2$. For each such entry we look for the row $t_{j,k}=?(t_j,t_k)$
and search for the base row $t_i$ and the scalar $\alpha$ for which  $t_{j,k} \treesColin{\alpha}{H} t_i$.
We get that $t_{1,2}\treesColin{1}{H} t_3$, $t_{3,2}\treesColin{0.5}{H} t_2$ and for all other $j,k$ we get $t_{j,k}\treesColin{1}{H} t_{4}$, so we set $c^{i}_{j,k}$ to be $0$ for every $i$. Thus, we obtain the following matrix for $\mu_{?}$
$$
\eta_{?}=\begin{bmatrix}0&0&0&0&0&0&0&0&0\\0&0&0&0&0&0&0&0.5&0\\
0&1&0&0&0&0&0&0&0\end{bmatrix}$$
% So $\mu_{?}(e_{1},e_{2})=e_{3}$ and $\mu(e_{3},e_{2})=0.5\cdot e_{1}$, and for every other combination of unit-basis vectors we obtain $\mu_{?}(e_{i},e_{j})=e_{1}$. 
 The vector $\lambda$ is also computed via Alg.~\AlgExtractCMTA, and we get $\lambda=(0,0,0.5)$. 
 
 The algorithm now asks an equivalence query and receives the following tree as a counter-example:
 
 $p=$\Tree [.? $a$ [.? [.? $a$ $b$ ] [.? [.? $a$ $b$ ] $b$ ] ] ]
 
 Indeed, while $\smq(p)=0$ we have that $\aut{A}(p)=0.125$. To see why $\aut{A}(p)=0.125$, let's look at the values $\mu(t)$ for every sub-tree $t$ of $p$. For the leaves, we have $\mu(a)=(1,0,0)$ and $\mu(b)=(0,1,0)$.
 
 Now, to calculate $\mu(?(a,b))$, we need to calculate $\mu_{?}(\mu(a),\mu(b))$. To do that, we first compose them as explained in Subsection.~\ref{subsec:multilinear}. The vector $P_{\mu(a),\mu(b)}$ is: $P_{\mu(a),\mu(b)}=(0,1,0,0,0,0,0,0,0)$. When multiplying this vector by the matrix $\eta_{?}$ we obtain $(0,0,1)$. So $\mu(?(a,b))=(0,0,1)$. Similarly, to obtain  $\mu(?(?(a,b),a))$ we first compose the value $(0,0,1)$
 for $?(a,b)$ with the value $(0,1,0)$ for $a$ and obtain $P_{\mu?(a,b),\mu(a)}=(0,0,0,0,0,0,0,1,0)$. 
 Then we multiply $\eta_{?}$ by $P_{\mu?(a,b),\mu(a)}$ and obtain $(0,0.5,0)$. In other words, 
 $$\mu(?(?(a,b),a))=\mu_{?}(\begin{bmatrix}0\\ 0\\ 1\end{bmatrix},\begin{bmatrix}0\\ 1\\ 0\end{bmatrix})=\begin{bmatrix}0\\0.5\\0\end{bmatrix}.$$ 
 
 The following tree depicts the entire calculation by marking the values obtained for each sub-tree. We can see that  $\mu(p)=(0,0,0.25)$, thus we get that $\aut{A}=\mu(p)\cdot\lambda=0.125$.
 
\vspace{2mm} 
 \scalebox{.9}{
   \Tree [.$(0,0,0.25)$ $(1,0,0)$ [.$(0,0.25,0)$ [.$(0,0,1)$ $(1,0,0)$ $(0,1,0)$ ] [.$(0,0.5,0)$ [.$(0,0,1)$ $(1,0,0)$ $(0,1,0)$ ] $(0,1,0)$ ] ] ]
}
\vspace{2mm} 

 We add all prefixes of this counter-example to $T$ and we obtain the following table:
 \begin{center}
 	\begin{tabular}{l | l | l | l | l }
 		 & & \Tree [.$\context$ ] & \rotatebox[origin=c]{90}{$?(a,\context)$} & \rotatebox[origin=c]{90}{$?(\context, b)$} \\ \hline
 		$t_1$ & $a$  & $0$ & $0$ & $\frac{1}{2}$ \\ \hline
 		$t_2$ & $b$ & $0$ & $\frac{1}{2}$ &$0$ \\ \hline
 		$t_3$ & $?(a,b)$ & $\frac{1}{2}$ & $0$ & $0$ \\\hline
 		$t_4$ & $?(a,a)$ & $0$ & $0$ & $0$\\\hline
 		$t_5$ & $?(?(a,a),a)$ & $0$ & $0$ & $0$\\\hline
 		$t_6$ & $?(?(a,b),b)$ & $0$ & $\frac{1}{4}$ & $0$ \\\hline
 		$t_7$ & $?(?(a,b),?(?(a,b),b))$ & $0$ & $0$ & $0$\\\hline
 		$t_8$ & $?(a,?(?(a,b),?(?(a,b),b)))$ & $0$ & $0$ & $0$ \\
 	\end{tabular}
 \end{center}
 This table is not consistent since while $t_6 \treesColin{0.5}{H} t_2$ this co-linearity is not preserved when extended with $t_{3}=?(a,b)$ to the left, as evident from the context $?(a,\context)$.
We thus add the context $\contextConcat{?(a,\context)}{?(?(a,b),\context)}=?(a,?(?(a,b),\context))$ to obtain the final table:

 \begin{center}
 	\begin{tabular}{l | l | l | l | l | l}
 		& & \Tree [.$\context$ ] & \rotatebox[origin=c]{90}{$?(a,\context)$} & \rotatebox[origin=c]{90}{$?(\context, b)$} & \rotatebox[origin=c]{90}{$?(a,?(?(a,b),\context))$}\\ \hline
 		$t_1$ & $a$ & $0$ & $0$ & $\frac{1}{2}$ & $0$\\ \hline
 		$t_2$ & $b$ & $0$ & $\frac{1}{2}$ & $0$ & $\frac{1}{4}$ \\ \hline
 		$t_3$ & $?(a,b)$ & $\frac{1}{2}$& $0$ & $0$ & $0$ \\\hline
 		$t_4$ & $?(a,a)$ & $0$ & $0$ & $0$ & $0$ \\\hline
 		  & $?(?(a,a),a)$ & $0$ & $0$ & $0$ & $0$ \\\hline
 		$t_5$ & $?(?(a,b),b)$ & $0$ & $\frac{1}{4}$ & $0$ & $0$ \\\hline
 		  & $?(?(a,b),?(?(a,b),b))$ & $0$ & $0$ & $0$ & $0$\\\hline
 		  & $?(a,?(?(a,b),?(?(a,b),b)))$ & $0$ & $0$ & $0$ & $0$ \\\hline
 		 $t_6$  & \color{blue}$?(a,?(?(a,b),b))$ & $\frac{1}{4}$  & $0$ & $0$ & $0$ \\
 	\end{tabular}
 \end{center}
 The table is now closed and consistent, and we extract the following CMTA from it: 
 $\aut{A}_3=(\Sigma,\mathbb{R},4,\mu,\lambda)$ with $\mu_{a}=(1,0,0,0)$, $\mu_{b}=(0,1,0,0)$. 
 Now $\mu_{?}$ is a $4\times 4^2$ matrix. Its interesting entries are $c^3_{1,2}=1$, $c^4_{3,2}=1$ and $c^3_{1,4}=\frac{1}{2}$
 since $t_{1,2}\treesColin{1}{H} t_3$, $t_{3,2} \treesColin{1}{H} t_5$, $t_{1,5} \treesColin{1}{H} t_6 \treesColin{0.5}{H} t_3$.
 And  for every other combination of unit-basis vectors we have $t_{i,j}\treesColin{1}{H} t_4$.   
 The final output vector is $\lambda=(0,0,0.5,0)$.
 
 The equivalence query on this CMTA returns true, hence the algorithm now terminates, and we can convert this CMTA into a WCFG. 
 Applying the transformation provided in Section.~\ref{sec:pmtawcfg} we obtain the following WCFG:
 \begin{align*}
 S&\longrightarrow N_{3}~[0.5]   \\
 N_{1}&\longrightarrow a~[1.0 ]  \\
 N_{2}&\longrightarrow b~[1.0]   \\
 N_{3}&\longrightarrow N_{1} N_{2}~[1.0]\ \  |\ \ N_{1} N_{4}~[0.5]   \\
 N_{4}&\longrightarrow N_{3} N_{2}~[1.0]  
 \end{align*}
 
 Now, following~\cite{abney1999relating,smith2007weighted}
 we can calculate the partitions functions for each non-terminal. Let $f_{N}$ be the sum of the weights of all trees whose root is $N$, we obtain:
 \begin{align*}
 f_{S}&=1\\
 f_{N_{1}}&=1\\
 f_{N_{2}}&=1\\
 f_{N_{3}}&=2\\
 f_{N_{4}}&=2\\
 \end{align*}
 
 Hence we obtain the PCFG 
 \begin{align*}
 S&\longrightarrow N_{3}~[1.0]\\
 N_{1}&\longrightarrow a~[1.0]\\
 N_{2}&\longrightarrow b~[1.0]\\
 N_{3}&\longrightarrow N_{1} N_{2}~[0.5]\ |\ N_{1} N_{4}~[0.5]\\
 N_{4}&\longrightarrow N_{3} N_{2}~[1.0]
 \end{align*}
 which is a correct grammar for the unknown probabilistic series.
 


==> pmta.tex <==

\begin{defi}
A positive multiplicity tree automaton (PMTA) is a multiplicity tree automaton (MTA) where all weights in both $\mu$ and $\lambda$ are positive. 
\end{defi}
PMTA are useful, since as we will soon show in Propositions \ref{prop:equiv1} and \ref{prop:equiv2}, PMTA can be converted to WCFG, and as shown by \cite{abney1999relating, smith2007weighted}, those can be converted to PCFGs. Hence, an algorithm for query learning of PMTA can be used for learning PCFGs.

\subsection{Equivalence of PMTA and WCFG}\label{sec:pmtawcfg}
Given a PMTA for a skeletal tree language, we can convert it to a WCFG.
Let $\mathcal{A}=(V=\mathbb{R}^{n},\mu,\lambda)$ be our PMTA, and $\Sigma=\bigcup_{k\geq 0}\Sigma_{(k)}$ be our skeletal alphabet, we will define a WCFG $\mathcal{G}_{\mathcal{A}}=(N,\Sigma_{0},R,S,W)$ in the following manner:
\begin{align*}
    N&=\{S\}\cup\{N_{i}:1\leq i\leq n\}\\
    R&=\{(S\rightarrow N_{i}):1\leq i\leq n\}\\
    &\cup\{(N_{i}\rightarrow N_{i_{1}}N_{i_{2}}...N_{i_{p}}):1\leq i \leq n, 1\leq i_{j}\leq n\text{ for } 1\leq j\leq p\}\\
    &\cup\{(N_{i}\rightarrow \sigma):1\leq i\leq n,\sigma\in\Sigma_{0}\}\\
    W(S\rightarrow N_{i})&=\lambda[i]\text{ for } 1\leq i\leq n\\
    W(N_{i}\rightarrow N_{i_{1}}N_{i_{2}}...N_{i_{p}})&=\mu(?)_{i,i_{1},i_{2},...,i_{p}} \text { for } 1\leq i \leq n, 1\leq i_{j}\leq n\text{ for } 1\leq j\leq p\\
    W(N_{i}\rightarrow\sigma)&=\mu(\sigma)_{i}\text{ for } 1\leq i\leq n, \sigma\in\Sigma_{0}\\
\end{align*}
\begin{prop}\label{prop:equiv1}
For each $t\in \Sigma_{T}$ we have that $W_{D(\mathcal{G}_{\mathcal{A}})}(t)=\mathcal{A}(t)$
\end{prop}
\begin{lem}\label{lemma:lemmasum}
Let $t=(?(t_{1},t_{2},...,t_{k}))\in \Sigma_{T}$. Then for each $i$:
\begin{equation*}
        \sum_{N_{j_{1}}N_{j_{2}}...N_{j_{k}}\in N^{k}} W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})W_{D_{N_{j_{1}}}(\mathcal{G})}(t_{1})\cdot...\cdot W_{D_{N_{j_{k}}}(\mathcal{G})}(t_{k})=W_{D_{N_{i}}(\mathcal{G})}(t)
\end{equation*}
\end{lem}
\begin{proof}[Proof of Lemma \ref{lemma:lemmasum}]
Consider a given sequence, $N_{j_{1}}N_{j_{2}}...N_{j_{k}}\in (N\cup\Sigma)^{k}$. Let's calculate the term:
\begin{equation*}
    W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})W_{D_{N_{j_{1}}}(\mathcal{G})}(t_{1})\cdot...\cdot W_{D_{N_{j_{k}}}(\mathcal{G})}(t_{k})
\end{equation*}
We claim that the value of this term is the sum of the weights of all parse trees in which the children of $t$ are labeled as $N_{j_{1}}N_{j_{2}}...N_{j_{k}}$.
For each $i$ s.t $N_{j_{i}}\in\Sigma$ $t_{i}$ must be labeled as $N_{j_{i}}$. Indeed, if $t_{i}\neq N_{j_{i}}$, then $W_{D_{N_{j_{i}}}}(t_{i})=0$ and the entire term equals zero. If $t_{i}= N_{j_{i}}$, then $W_{D_{N_{j_{i}}}}(t_{i})=1$ and the term is not affected by $t_{i}$.
Now, for all $i$ s.t $N_{j_{i}}\notin\Sigma$ we have that $W_{D_{N_{j_{i}}}}(t_{i})$ is equal to the sum of all trees in $D_{N_{j_{i}}}$ with the skeleton $t_{i}$.
All those trees, by definition, have $N_{j_{i}}$ as their root. So:
\begin{equation*}
    W_{D_{N_{j_{i}}}}(t_{i})=\sum_{t'_{i}\in D_{N_{j_{i}}}} W(t'_{i})
\end{equation*}
Let $D_{N_{j_{i}}}=\{t_{i_{1}},t_{i_{2}},...,t_{i{|D_{N_{j_{i}}}|}}\}$

We have then:
\begin{align*}
    &W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})W_{D_{N_{j_{1}}}(\mathcal{G})}(t_{1})\cdot...\cdot W_{D_{N_{j_{k}}}(\mathcal{G})}(t_{k})\\
    &=W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})\sum_{t'\in D_{N_{j_{1}}}} W(t'_{1})\cdot...\cdot \sum_{t'_{k}\in D_{N_{j_{k}}}} W(t'_{k})\\
    &=W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})t_{1_{1}}\cdot...\cdot t_{k_{1}}+
    W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})t_{1_{1}}\cdot...\cdot t_{k_{2}}+...\\
    &+W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})t_{1_{|D_{N_{j_{1}}}|}}\cdot...\cdot t_{k_{|D_{N_{j_{k}}}|}}
\end{align*}
One can observe that we multiply all possible combinations of trees from each set $D_{N_{j_{i}}}$ by the production weight $W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})$. By definition of $W':D(\mathcal{G})\rightarrow\mathbb{R}$, we have that each element in the sum is a weight of a tree in $D_{N_{i}}(\mathcal{G})$. So the resulting sum is the sum of the weight of all the trees in which the children are labeled as $N_{j_{1}}N_{j_{2}}...N_{j_{k}}$.

Notice that in our original sum, we go over all possible sequences of labels for the children, so it follows that we go over all trees in $D_{N_{i}}(\mathcal{G})$. So:
\begin{equation*}
        \sum_{N_{j_{1}}N_{j_{2}}...N_{j_{k}}\in N^{k}} W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{k}})W_{D_{N_{j_{1}}}(\mathcal{G})}(t_{1})\cdot...\cdot W_{D_{N_{j_{k}}}(\mathcal{G})}(t_{k})=W_{D_{N_{i}}(\mathcal{G})}(t)
\end{equation*}
\end{proof}
\begin{proof}[Proof of Proposition \ref{prop:equiv1}]
We will first prove the following claim:

Let $t\in \Sigma_{T}$, the vector $v=(v_{1},v_{2},...,v_{n})$ calculated by $\mathcal{A}$ for the root of the tree maintains that for each $i$, $v_{i}=W_{D_{N_{i}}(\mathcal{G}_{\mathcal{A}})}(t)$.
We will prove by induction on the height of $t$. \textbf{Base case:} $h=1$. Then $t$ is a leaf, so $t\in\Sigma$. Then for each $i$ we have that $v[i]=\mu(\sigma)_{i}$. By our definition of $\mathcal{G}_{\mathcal{A}}$ we have $W(N_{i}\rightarrow\sigma)=\mu(\sigma)_{i}$ for each $i$ and for each $\sigma\in\Sigma$, so the claim holds. \textbf{Induction step:} $h>1$. Then $t=(?(t_{1},t_{2},...,t_{k}))$. For each $i$ let $v_{i}$ be the vector calculated by $\mathcal{A}$ for $t_{i}$. By the definition of a multi-linear map, for each $i$ we have:
\begin{equation*}
        v[i]=\sum_{1\leq j_{i}\leq d} \mu(?)_{i,j_{1},...,j_{p}}v_{i}[j_{1}]\cdot...\cdot v_{p}[j_{p}]
\end{equation*}
By our definition of $\mathcal{G}_{\mathcal{A}}$ we have that $\mu(?)_{i,j_{1},...,j_{p}}=W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{p}})$. Also, from our induction hypothesis, we have that for each $j_{i}$, $v_{i}[j_{i}]=W_{D_{N_{j_{i}}}(\mathcal{G}_{\mathcal{A}})}(t_{i})$ So we have that:
\begin{equation*}
        v[i]=\sum_{N_{j_{1}}N_{j_{2}}...N_{j_{p}}\in N^{p}} W(N_{i}\rightarrow N_{j_{1}}N_{j_{2}}...N_{j_{p}})W_{D_{N_{j_{1}}}(\mathcal{G}_{\mathcal{A}})}(t_{1})\cdot...\cdot W_{D_{N_{j_{p}}}(\mathcal{G}_{\mathcal{A}})}(t_{p})
\end{equation*}
Which according to Lemma \ref{lemma:lemmasum} is equal to $W_{D_{N_{i}}(\mathcal{G}_{\mathcal{A}})}(t)$ as required.
Now let $t\in K(D(\mathcal{G}_{\mathcal{A}}))$. Let $v=(v_{1},v_{2},...,v_{n})$ be the vector calculated by $\mathcal{A}$ for $t$. 
The value calculated by $\mathcal{A}$ is $\lambda\cdot v$, which is:
\begin{equation*}
    \sum_{i=1}^{n} v_{i}\cdot \lambda[i]
\end{equation*}
By our definition of $\mathcal{G}_{\mathcal{A}}$ we have that $\lambda[i]=W(S\rightarrow N_{i})$ for each $i$. So we have:
\begin{equation*}
    \sum_{i=1}^{n} v_{i}\cdot \lambda[i] = W(S\rightarrow N_{i})\cdot v_{i}
\end{equation*}
By our claim, for each $i$, $v_{i}$ is equal to the probability of deriving $t$ starting from the non-terminal $N_{i}$, so we have that the value calculated by $\mathcal{A}$ is the probability of deriving the tree starting from the start symbol $S$. That is, for each $t\in K(D(\mathcal{G}_{\mathcal{A}}))$, $W_{D(\mathcal{G}_{\mathcal{A}})}(t)=\mathcal{A}(t)$.
\end{proof}
\subsubsection{Converting a WCFG into a PMTA}
Let $\mathcal{G}=(N,\Sigma,R,S,W)$ be a WCFG. Suppose w.l.o.g that $N=\{N_{0},N_{1},...,N_{|N|-1}\}$, $\Sigma=\{\sigma_{0},\sigma_{1},...,\sigma_{|\Sigma|-1}\}$ and that $S=N_{0}$. Let $n=|N|+|\Sigma|$. We'll define a function $\iota:N\cup\Sigma\rightarrow\mathbb{N}_{\leq n}$ in the following manner:
\[
\iota(x) =
\begin{dcases*}
j
   & $x=N_{j}\in N$\\
   |N|+j
   & $x=\sigma_{j}\in \Sigma$
\end{dcases*}
\]
Note that since $N\cap\Sigma=\emptyset$, $\iota$ is well defined. Also, it's easy to observe that $\iota$ is a bijection, so $\iota^{-1}:\mathbb{N}_{\leq n}\rightarrow N\cup\Sigma$ is also a function.

We'll define a PMTA $\mathcal{A}_{\mathcal{G}}$ in the following manner:
\begin{equation*}
    \mathcal{A}_{\mathcal{G}}=(V=\mathbb{R}^{n},\mu,\lambda)
\end{equation*}
Where:
\begin{equation*}
    \lambda=[1,0,...,0]
\end{equation*}
That is, $\lambda[0]=1$, and for $1<i\leq n$ $\lambda[i]=0$.\\
For each $\sigma\in\Sigma$:

\[
\mu(\sigma)_{i} =
\begin{dcases*}
1
   & $i=\iota(\sigma)$\\
   0
   & otherwise
\end{dcases*}
\]
We define $\mu(?)$ in the following way:
\[
\mu(?)_{i,i_{1},i_{2},...,i_{j}} =
\begin{dcases*}
W(\iota^{-1}(i)\rightarrow \iota^{-1}(i_{1})\iota^{-1}(i_{2})...\iota^{-1}(i_{j}))
   & $1\leq i\leq |N|$\\
   0
   & otherwise
\end{dcases*}
\]
\begin{exa}
Let $\mathcal{G}=(N,\Sigma,R,S,W)$ be the following WCFG, with $N=\{S\}$, $\Sigma=\{a,b\}$ $R=\{S\rightarrow aSb, S\rightarrow ab\}$ and $W(S\rightarrow aSb)=0.6$ and $W(S\rightarrow ab)=0.4$. So for example $W(ab)=0.4$, $W(aabb)=0.24$ and generally: $W(a^{n}b^{n})=0.4\cdot 0.6^{n-1}$.\\
The function $\iota$ would be: $\iota(S)=0$, $\iota(a)=1$, $\iota(b)=2$.
By our conversion the equivalent PMTA would be:
\begin{equation*}
    \mathcal{A}_{\mathcal{G}}=(V=\mathbb{R}^{3},\mu,\lambda)
\end{equation*}
$\lambda=(1,0,0)$, $\mu(a)=(0,1,0)$, $\mu(b)=(0,0,1)$.\\
$\mu(?)_{0,1,2}=0.4$ since $W(S\rightarrow ab)=0.4$, and $\mu(?)_{0,1,0,2}=0.6$ since $W(S\rightarrow aSb)$.

Consider the following tree:
\begin{center}
\Tree[.? a [.? a b ] b ]
\end{center}

The MTA would work on it in a bottom-up manner. We mark values calculated by the MTA in blue in the respective node in the tree. Since $\mu(a)=(0,1,0)$ and $\mu(b)=(0,0,1)$ we have:

\begin{center}

\Tree[.? a [.? \color{blue}(0,1,0) \color{blue}(0,0,1) ] b ]
\end{center}
Now we calculate $\mu(?)((0,1,0),(0,0,1))$. Since $\mu(?)_{0,1,2}=0.4$ and for all other values $\mu(?)_{i,i_{1},i_{2}}=0$ we have:

\begin{center}
\Tree[.? \color{blue}(0,1,0) [.\color{blue}(0.4,0,0) \color{blue}(0,1,0) \color{blue}(0,0,1) ] \color{blue}(0,0,1) ]
\end{center}
Now we calculate $\mu(?)((0,1,0),(0.4,0,0),(0,0,1))$. Since $\mu(?)_{0,1,0,2}=0.6$ and for all other values $\mu(?)_{i,i_{1},i_{2},i_{3}}=0$ we have:

\begin{center}
\Tree[.\color{blue}(0.24,0,0) \color{blue}(0,1,0) [.\color{blue}(0.6,0,0) \color{blue}(0,1,0) \color{blue}(0,0,1) ] \color{blue}(0,0,1) ]
\end{center}
The end result is $\lambda\cdot (0.24,0,0)=0.24$. 
\end{exa}
\begin{prop}\label{prop:equiv2}
For each $t\in K(D(\mathcal{G}))$ we have that $W_{D(\mathcal{G})}(t)=\mathcal{A}_{\mathcal{G}}(t)$
\end{prop}
\begin{proof}
The proof would be similar to the proof of Proposition \ref{prop:equiv1}.

We will first prove by induction that for each $t\in K(D(\mathcal{G}))$ the vector $v=(v[1],v[2],...,v[n])$ calculated by $\mathcal{A}_{\mathcal{G}}$ maintains that for each $i\leq |N|$, $v[i]=W_{D_{N_{i}}(\mathcal{G})}$, and for $i>|N|$ $v[i]=1$ iff $t=\iota^{-1}(i)$ and $v[i]=0$ otherwise.

Proof by induction on the height of $t$. \textbf{Base:} $h=1$, then $t$ is a leaf, so $t=\sigma\in\Sigma$. By definition $\mu(\sigma)_{i}=1$ if $i=\iota(\sigma)$ and $0$ otherwise. So $v[\iota(\sigma)]=1$, and for every $i\neq\iota(\sigma)$ $v[i]=0$. Since the root of the tree is in $\Sigma$, the root of the tree can't be a non-terminal, so $W_{D_{N_{i}}(\mathcal{G})}=0$ for every $i$. So the claim holds. \textbf{Induction step:} $h>1$, then $t=(? (t_{1}, t_{2},...,t_{k}))$. Let $v=(v[1],v[2],...,v[n])$ be the vector calculated by $\mathcal{A}$ for $t$. By our definition of $\mu(?)$, for every $i>|N|$ $\mu(?)_{i,i_{1},i_{2},...,i_{j}}=0$ for all values of $i_{1},i_{2},...,i_{j}$. So for every $i>|N|$ we have that $v[i]=0$ as required, since $t\notin\Sigma$. Now for $i\leq|N|$. By definition of a multi-linear map we have that:
\begin{equation*}
        v[i]=\sum_{1\leq j_{i}\leq d} \mu(?)_{i,j_{1},...,j_{p}}v_{1}[j_{1}]\cdot...\cdot v_{p}[j_{p}]
\end{equation*}
Since $i\leq |N|$, by our definition we have that:
\begin{equation*}
    \mu(?)_{i,j_{1},...,j_{p}}=W(\iota^{-1}(i)\rightarrow \iota^{-1}(j_{1})\iota^{-1}(j_{2})...\iota^{-1}(j_{p}))
\end{equation*}
For each $j_{k}$ let $B_{k}=\iota^{-1}(j_{k})$, also since $i\leq |N|$, $\iota^{-1}(i)=N_{i}$, so:
\begin{equation*}
    \mu(?)_{i,j_{1},...,j_{p}}=W(N_{i}\rightarrow B_{1}B_{2}...B_{j})
\end{equation*}
For each $i$, by our induction hypothesis, if $t_{i}$ is a leaf, $v_{i}[j_{i}]=1$ only for $j_{i}=\iota(t_{i})$, and otherwise $v_{i}[j_{i}]=0$. If $t_{i}$ isn't a leaf, then for every $j_{i}>|N|$ $v_{i}[j_{i}]=0$, and for $j_{i}\leq |N|$, we have that $v_{i}[j_{i}]=W_{D_{N_{j_{i}}}(\mathcal{G})}$. So we have:
\begin{equation*}
        v[i]=\sum_{1\leq j_{i}\leq d} W(N_{i}\rightarrow B_{1}B_{2}...B_{j})W_{D_{N_{j_{1}}}(\mathcal{G})}\cdot...\cdot W_{D_{N_{j_{p}}}(\mathcal{G})}
\end{equation*}
So by lemma \ref{lemma:lemmasum} we have that $v[i]=W_{D_{N_{i}}(\mathcal{G})}$ as required.\\
Now let $t\in K(D(\mathcal{G}))$. Let $v=(v_{1},v_{2},...,v_{n})$ be the vector calculated by $\mathcal{A}_{\mathcal{G}}$ for $t$. 
By our claim, for each $i\leq |N|$, $v_{i}=W_{D_{N_{i}}(\mathcal{G})}$, since $S=N_{0}$, we have that $v[1]=W_{D_{S}(\mathcal{G})}$. Also, since $\lambda=(1,0,...,0)$ we have that $\mathcal{A}_{\mathcal{G}}(t)$ is $v[1]$, which is $W_{D_{S}(\mathcal{G})}=W_{D(\mathcal{G})}(t)$. So it follows that for every $t\in K(D(\mathcal{G}))$ $W_{D(\mathcal{G})}(t)=\mathcal{A}_{\mathcal{G}}(t)$. 
\end{proof}
\subsection{Trying to accommodate M* for learning PMTA}\label{sec:mstarpmta}
In this section we prove two propositions, which show that one cannot use \mstar algorithm to learn PMTA. Proposition \ref{prop:mstar_negative_mta} shows a grammar, for which there exist a PMTA, and a positive base in the Hankel Matrix, but applying \mstar algorithm as is may choose a non negative base.

In Proposition.\ref{prop:mstar_always_returns_non_positive} shows that there are grammars which have PMTA, but since their respective Hankel Matrices do not contain a positive base, \mstar\ would always return a non-positive MTA.
\begin{prop}\label{prop:mstar_negative_mta}
There exists a probabilistic word series for which the \mstar\ algorithm may return an MTA with negative weights.
\end{prop}

\begin{proof}
    Let $\mathcal{G}$ be the grammar that assigns to the words $aa$,$ab$,$ac$,$ba$,$cb$,$cc$ a probability of $\frac{1}{6}$ and to all other words a probability of $0$. For simplicity we assume that the grammar is regular.
	The first rows of Hankel Matrix for this word series are given in the Figure.\ref{fig:mta_non_positive} (all entries not in the figure are $0$).
	One can see that the rows $\epsilon$, $b$, $c$, $ba$ are a positive span of the entire Hankel Matrix. 
	However, the $\mstar$ algorithm may return the MTA spanned by the basis $\epsilon$, $a$, $b$, $aa$. 
	Since the row of $c$ is obtained by subtracting the row of $b$ from the row of $a$, this MTA will contain negative weights.
	
\begin{figure}
    \centering
        \begin{tabular}{ c|c|c|c|c|c|c|c|c|c|c|c|c|c } 
  & $\varepsilon$ & $a$ & $b$ & $c$& $aa$ & $ab$ &$ac$& $ba$& $bb$& $bc$& $ca$ &$cb$& $cc$\\ \hline
  
 \diagfil{2cm}{gray!50}{gray!25}{$\varepsilon$}& $0$ & $0$ & $0$ & $0$&$\frac{1}{6}$&$\frac{1}{6}$&$\frac{1}{6}$&$\frac{1}{6}$&$0$&$0$&$0$&$\frac{1}{6}$&$\frac{1}{6}$ \\ \hline 
 \cellcolor{gray!50} $a$ & $0$ & $\frac{1}{6}$ & $\frac{1}{6}$ & $\frac{1}{6}$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\ \hline
 \diagfil{2cm}{gray!50}{gray!25}{$b$} & $0$ & $\frac{1}{6}$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$\\ \hline
 \cellcolor{gray!25} $c$ & $0$ & $0$ & $\frac{1}{6}$ & $\frac{1}{6}$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$\\ \hline
 \cellcolor{gray!50} $aa$ & $\frac{1}{6}$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\  \hline
 $ab$ & $\frac{1}{6}$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\  \hline
 $ac$ & $\frac{1}{6}$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\  \hline
 $ba$ & $\frac{1}{6}$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$\\ \hline
 $bb$ & $0$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\  \hline
 $bc$ & $0$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$\\  \hline
 $ca$ & $0$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\  \hline
 \cellcolor{gray!25}$cb$ & $\frac{1}{6}$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\ \hline
 $cc$ & $\frac{1}{6}$ & $0$ & $0$ & $0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$&$0$ \\
\end{tabular}
    \caption{The observation table for the grammar $\mathcal{G}$. Two of the possible bases are highlighted. The red one results in a negative MTA, while the orange one results in a positive one, that can be converted to a PCFG. For simplicity, the trees are presented as words, since we assume that the grammar is regular.}
    \label{fig:mta_non_positive}
\end{figure}
\end{proof}
In Proposition \ref{prop:mstar_always_returns_non_positive} we show that there exists a PCFG $\grmr{G}$ such that the Hankel Matrix
	$H_\grmr{G}$ corresponding to its tree-series $\treesrs{T}_G$ has the property that
	no finite number of rows spans the entire matrix.
Before proving Proposition \ref{prop:mstar_always_returns_non_positive}, we prove the following lemma:
\begin{lem}\label{lemmaSing}
	Let $B=\{b_{1},b_{2},...,b_{p}\}$ be set of positively independent vectors. 
	Let $\hat{B}$ be a matrix whose rows are the elements of $B$, and let $\alpha$ be a positive vector. 
	Then if $\hat{B}\alpha=b_{i}$ then $\alpha[i]=1$ and $\alpha[j]=0$ for every $j\neq i$.
\end{lem}

\begin{proof}
	Assume $b_{i}=\hat{B}\alpha$. Then we have:
	\begin{equation*}
	    b_{i}=\hat{B}\alpha=\sum_{j=1}^{p}\alpha_{j}b_{j}=\alpha_{i}b_{i}+\sum_{j\neq i}\alpha_{j}b_{j}
	\end{equation*}
	If $\alpha_{i}<1$ we obtain:
	\begin{equation*}
	    b_{i}(1-\alpha_{i})=\sum_{j\neq i}\alpha_{j}b_{j}
	\end{equation*}
	Which is a contradiction, since $b_{i}\in B$ and thus can't be described as a positive combination of the other elements.
	
	If $\alpha_{i}>1$ we obtain:
	\begin{equation*}
	    \sum_{j\neq i}\alpha_{j}b_{j}+(\alpha_{i}-1)b_{i}=0
	\end{equation*}
	This is a contradiction, since each $b>0$, and each $\alpha_{j}\geq 0$, with $\alpha_{i}>1$.
	
	Hence $\alpha_{i}=1$. Therefore we have:
	\begin{align*}
	    \sum_{j\neq i}\alpha_{j}b_{j}=0
	\end{align*}
	Since $\alpha_{j}\geq 0$, and $b_{j}>0$ the only solution is that $\alpha_{j}=0$ for every $j\neq i$.
\end{proof}

\begin{prop}\label{prop:mstar_always_returns_non_positive}
There exists a PCFG $\grmr{G}$ such that the Hankel Matrix
	$H_\grmr{G}$ corresponding to its tree-series $\treesrs{T}_G$ has the property that
	no finite number of rows spans the entire matrix.
\end{prop}

\begin{proof}
Let $\grmr{G}=(\{a\},\{N_{1},N_{2}\},R,N_{1})$ be the following PCFG:
$$\begin{array}{l@{\ \longrightarrow\ }l}
N_{1}& aN_{1}~[\frac{1}{2}]\ \mid\  aN_{2}~[\frac{1}{3}]\ \mid\  aa~[\frac{1}{6}]\\[2mm]
N_{2}& aN_{1}~[\frac{1}{4}]\ \mid\  aN_{2}~[\frac{1}{4}]\ \mid\  aa~[\frac{1}{2}]
\end{array}$$

We say that a tree has a \emph{chain structure} if every inner node is of branching-degree $2$ and has
one child which is a terminal. We say that a tree has a \emph{right-chain structure} (resp. \emph{left-chain structure})
if the non-terminal is always the right (resp. left) child.
Note that all trees in $\sema{G}$ have a right-chain structure (and the terminals are always the letter $a$), and can
be depicted as follows:

\Tree [.? $a$ [.? $a$ [.$\ddots$ $a$ [.? $a$ $a$ ] ] ] ]\vspace{2mm}

Let us denote by $p_{n}$ the total probability of all trees with $n$ non-terminals s.t. the lowest non terminal is $N_{1}$, 
and similarly, let us denote by $q_{n}$ the total probability of all trees with $n$ non-terminals s.t. the lowest non-terminal is $N_{2}$. 

We have that $p_{0}=0$, $p_{1}=\frac{1}{6}$, and  $p_{2}=\frac{1}{12}$. We also have that $q_{0}=0$, $q_{1}=0$ and  $q_{2}=\frac{1}{6}$. 

Now, to create a tree with $n$ non-terminals, we should take a tree with $n-1$ non-terminals, ending with either $N_{1}$ or $N_{2}$, and use the last derivation. So we have:
\begin{align*}
p_{n}&=\frac{1}{2}\cdot p_{n-1}+\frac{1}{4}\cdot q_{n-1}\\
q_{n}&=\frac{1}{3}\cdot p_{n-1}+\frac{1}{4}\cdot q_{n-1}
\end{align*}

We want to express $p_{n}$ only as a function of $p_{i}$ for $i<n$, and similarly for $q_{n}$. Starting with the first equation we obtain:
\begin{align*}
p_{n}&=\frac{1}{2}\cdot p_{n-1}+\frac{1}{4}\cdot q_{n-1}\\
4\cdot p_{n+1}-2\cdot p_{n}&=q_{n}\\
4\cdot p_{n}-2\cdot p_{n-1}&=q_{n-1}
\end{align*}

And from the second equation we obtain:
\begin{align*}
q_{n}&=\frac{1}{3}\cdot p_{n-1}+\frac{1}{4}\cdot q_{n-1}\\
3\cdot q_{n+1}-\frac{3}{4}\cdot q_{n}&=p_{n}\\
3\cdot q_{n}-\frac{3}{4}\cdot q_{n-1}&=p_{n-1}
\end{align*}

Now setting these values in each of the equation, we obtain:

\begin{align*}
4\cdot p_{n+1}-2\cdot p_{n}&=\frac{1}{3}\cdot p_{n-1}+\frac{1}{4}(4\cdot p_{n}-2\cdot p_{n-1})\\
p_{n+1}&=\frac{1}{2}\cdot p_{n}+\frac{1}{12}\cdot p_{n-1}+\frac{1}{16}(4\cdot p_{n}-2\cdot p_{n-1})\\
p_{n+1}&=\frac{1}{2}\cdot p_{n}+\frac{1}{12}\cdot p_{n-1}+\frac{1}{4}\cdot p_{n}-\frac{1}{8}\cdot p_{n-1}\\
p_{n+1}&=\frac{3}{4}\cdot p_{n}-\frac{1}{24}\cdot p_{n-1}
\end{align*}

And:

\begin{align*}
3\cdot q_{n+1}-\frac{3}{4}\cdot q_{n}&=\frac{1}{2}\cdot(3\cdot q_{n}-\frac{3}{4}\cdot q_{n-1})+\frac{1}{4}\cdot q_{n-1}\\
3\cdot q_{n+1}&=\frac{9}{4}\cdot q_{n}-\frac{1}{8}\cdot q_{n-1}\\
q_{n+1}&=\frac{9}{12}\cdot q_{n}-\frac{1}{24}\cdot q_{n-1}=\frac{3}{4}\cdot q_{n}-\frac{1}{24}\cdot q_{n-1}
\end{align*}
Let's denote by $t_{n}$ the probability that $\mathcal{G}$ assigns to $a^{n}$. This probability is:
\begin{equation*}
t_{n}=\frac{1}{6}\cdot p_{n-1}+\frac{1}{2}\cdot q_{n-1}
\end{equation*}
Since $$p_{n-1}=\frac{3}{4}\cdot p_{n-2}-\frac{1}{24}\cdot p_{n-3}$$ and $$q_{n-1}=\frac{3}{4}\cdot q_{n-2}-\frac{1}{24}\cdot q_{n-3}$$ we obtain:
{\small
\begin{align*}
t_{n}=&\frac{1}{6}\cdot(\frac{3}{4}\cdot p_{n-2}-\frac{1}{24}\cdot p_{n-3})+\frac{1}{2}\cdot(\frac{3}{4}\cdot q_{n-2}-\frac{1}{24}\cdot q_{n-3})\\
t_{n}=&\frac{1}{6}\cdot\frac{3}{4}\cdot p_{n-2}-\frac{1}{6}\cdot\frac{1}{24}\cdot p_{n-3}+\frac{1}{2}\cdot\frac{3}{4}\cdot q_{n-2}-\frac{1}{2}\cdot\frac{1}{24}\cdot q_{n-3}\\
t_{n}=&\frac{3}{4}\cdot(\frac{1}{6}\cdot p_{n-2}+\frac{1}{2}\cdot q_{n-2})-\frac{1}{24}\cdot(\frac{1}{6}\cdot p_{n-3}+\frac{1}{2}\cdot q_{n-3})=\\
       =&\frac{3}{4}\cdot t_{n-1}-\frac{1}{24}\cdot t_{n-2}
\end{align*}
}

Hence, overall, we obtain:
\begin{equation*}
t_{n}=\frac{3}{4}\cdot t_{n-1}-\frac{1}{24}\cdot t_{n-2}
\end{equation*}

Now, let $L$ be the skeletal-tree-language of the grammar $\mathcal{G}$, and let $H$ be the Hankel Matrix for this tree set. Note, that any tree $t$ whose structure is not a right-chain, would have $L(t)=0$, and also for every context $c$, $L(\contextConcat{c}{t})=0$. Similarly, every context $c$ who violates the right-chain structure, would have $L(\contextConcat{c}{t})=0$ for every $t$.

Let $T_{n}$ be the skeletal tree for the tree of right-chain structure, with $n$ leaves. We have that $L(T_{1})=0$, $L(T_{2})=\frac{1}{6}$, $L(T_{3})=\frac{1}{4}$, and for every $i>3$ we have $$L(T_{i})=\frac{3}{4}\cdot L(T_{i-1})-\frac{1}{24}\cdot L(T_{i-2}).$$ Let $v_{i}$ be the infinite row-vector of the Hankel matrix corresponding to $T_{i}$. We have that for every $i>3$, $$v_{i}=\frac{3}{4}\cdot v_{i-1}-\frac{1}{24}\cdot v_{i-2}.$$ Assume towards contradiction that there exists a subset of rows that is a positive base and spans the entire matrix $H$.

Let $B$ be the positive base, whose highest member (in the lexicographic order) is the lowest among all the positive bases. Let $v_{r}$ be the row vector for the highest member in this base. Thus, $v_{r+1}\in\posspan{B}$. Hence:
\begin{equation*}
v_{r+1}=\alpha \hat{B}
\end{equation*}
Also, $v_{r+1}=\frac{3}{4}\cdot v_{r}-\frac{1}{24}\cdot v_{r-1}$. Therefore,
\begin{align*}
\frac{3}{4}\cdot v_{r}-\frac{1}{24}\cdot v_{r-1}=\alpha\hat{B}\\
v_{r}=\frac{4}{3}\cdot\alpha\hat{B}+\frac{1}{18}\cdot v_{r-1}
\end{align*}

We will next show that $v_{r-1}$ and $v_r$ are co-linear, which contradicts our choice of $v_r$.
Since $v_{r-1}\in\posspan{B}$ we know $v_{r-1}=\alpha'\hat{B}$ for some $\alpha'$. Therefore, 
\begin{equation*}
v_{r}=(\frac{4}{3}\cdot\alpha+\frac{1}{18}\cdot\alpha')\hat{B}
\end{equation*}
Let $\beta=\frac{4}{3}\cdot\alpha+\frac{1}{18}\cdot\alpha'$. Since $\alpha$ and $\alpha'$ are non-negative vectors, so is $\beta$. And by lemma \ref{lemmaSing}  it follows that for every $i\neq r$:
\begin{equation*}
\beta_{i}=\frac{4\cdot\alpha_{i}}{3}+\frac{\alpha'_{i}}{18}=0
\end{equation*}
Since $\alpha_{i}$ and $\alpha'_{i}$ are non-negative, we have that $\alpha_{i}=\alpha'_{i}=0$.

Since for every $i\neq r$, $\alpha'_{i}=0$, it follows that $v_{r-1}=m\cdot v_{r}$ for some $m\in\mathbb{R}$. 
Now, $m$ can't be zero since our language is strictly positive and all entries in the matrix are non-negative. Thus, $v_{r}=\frac{1}{m}\cdot v_{r-1}$, and $v_{r}$ and $v_{r-1}$ are co-linear. We can replace $v_{r}$ by $v_{r-1}$, contradicting the fact that we chose the base whose highest member is as low as possible.
\end{proof}

==> preliminaries.tex <==
We start by introducing some necessary definitions.
\subsection{Context Free Grammars (CFG), Weighted CFGs and Probabilistic CFGs}\label{sec:cfg}
We start with the standard definition of a context-free grammar. 

\subsubsection{Context Free Grammar}

	A \emph{context free grammar} (CFG) is a $4$-tuple $\grmr{G}=\langle \Vars,\Sigma,R,S\rangle$, where:
	\begin{itemize}
	    \item $\Vars$ is a finite non-empty set of symbols called  \emph{variables} or \emph{non-terminals}.
	    \item $\Sigma$ is a finite non-empty set of symbols called the \emph{alphabet} or the \emph{terminals}.
	    \item $R\subseteq \Vars\times (\Vars\cup\Sigma)^{*}$ is a relation between variables and strings over $\Vars\cup\Sigma$, called the  \emph{production rules}. 
	    \item $S\in \Vars$ is a special variable called the \emph{start variable}.
	\end{itemize}
As usual, if $(N,w)\in R$ we write $N\derives w$.	
\subsubsection{Derivation Trees}
A derivation tree is a rooted tagged tree, whose root is tagged with the start symbol of the grammar, its leaves are tagged with some terminal symbols, its inner nodes are tagged with non-terminal symbols, and for every inner node in the tree, if its tag is $N\in\Vars$, and the tags of its children are $t_{1},t_{2},\dots,t_{k}$ then $N\rightarrow t_{1}t_{2}\dots t_{k}$.

\commentout{
\begin{exa}
Let $\mathcal{G}=\langle \Vars,\Sigma,R,S\rangle$ be the grammar with: $\Vars=\{S,N_{1},N_{2}\}$, $\Sigma=\{a,b\}$, $R=\{(S,N_{1}),(S,N_{2}),(N_{1},aN_{1}),(N_{1},a),(N_{2},b)\}$. We can describe this grammar concisely using the following notation:
\begin{align*}
    \hspace{2.1cm}
    S&\derives N_{1}\mid N_{2}\\
    N_{1}&\derives a\; N_{1}\mid a\\
    N_{2}&\derives b
\end{align*}
An illustration of three possible derivation trees that can be derived from this grammar is available in Figure.\ref{fig:derivationTrees}.
\end{exa}}

\commentout{
\begin{figure}
\centering
\noindent\makebox[\textwidth]{
\begin{minipage}{.3\textwidth}
\begin{tikzpicture}
\end{tikzpicture}
\end{minipage}%
\begin{minipage}{.2\textwidth}
        \begin{tikzpicture}
            \node[shape=circle,draw=none] (A1) at (0,2) {$S$};
                \node[shape=circle,draw=none] (A2) at (0,1) {$N_{1}$};
                \path [-] (A1) edge node[right] {} (A2);
                \node[shape=circle,draw=none] (A3) at (0,0) {$a$};
                \path [-] (A2) edge node[right] {} (A3);    
        \end{tikzpicture}
\end{minipage}%
\begin{minipage}{.3\textwidth}
    \begin{tikzpicture}
        \node[shape=circle,draw=none] (B1) at (0,3) {$S$};
        \node[shape=circle,draw=none] (B2) at (0,2) {$N_{1}$};
        \path [-] (B1) edge node[right] {} (B2);
        \node[shape=circle,draw=none] (B3) at (1,1) {$N_{1}$};
        \node[shape=circle,draw=none] (B4) at (-1,1) {$a$};
        \path [-] (B2) edge node[right] {} (B3);
        \path [-] (B2) edge node[right] {} (B4);
        \node[shape=circle,draw=none] (B5) at (1,0) {$a$};
        \path [-] (B3) edge node[right] {} (B5);
    \end{tikzpicture}
\end{minipage}%
\begin{minipage}{.2\textwidth}
    \begin{tikzpicture}
        \node[shape=circle,draw=none] (C1) at (0,2) {$S$};
        \node[shape=circle,draw=none] (C2) at (0,1) {$N_{2}$};       
        \path [-] (C1) edge node[right] {} (C2);
        \node[shape=circle,draw=none] (C3) at (0,0) {$b$};      
        \path [-] (C2) edge node[right] {} (C3);
    \end{tikzpicture}
\end{minipage}%
\begin{minipage}{.3\textwidth}
\begin{tikzpicture}
\end{tikzpicture}
\end{minipage}%
}
\caption{Derivation trees}
\label{fig:derivationTrees}
\end{figure}
}


\subsubsection{Weighted Context Free Grammar}
A \emph{weighted context free grammar}  (WCFG) is a pair $\tuple{\grmr{G},\theta}$ where $\grmr{G}=\langle \Vars,\Sigma,R,S\rangle$ is a CFG and $\theta:R\rightarrow \R$ is a function mapping each production rule to a weight in $\R$.
A WCFG $\grmr{W}=\tuple{\grmr{G},\theta}$ defines a function from words over $\Sigma$ to weights in $\R$. 
The WCFG associates with a derivation tree $t$ its weight, which is defined as:
\begin{equation*}
    \grmr{W}(t)=\prod_{(V\derives \alpha)\in R } \theta(V\derives\alpha)^{\sharp_t(V\derives\alpha)}
\end{equation*}
Where $\sharp_t(V\derives\alpha)$ is the number of occurrences of the production $V\derives\alpha$ in the derivation tree $t$.


We abuse notation and treat $\semagrmr{\grmr{W}}$ also as a function from $\Sigma^*$ to $\R$  defined as %follows. 
$\grmr{W}(w)=\sum_{S\transderives{t}w}\grmr{W}(t)$.
That is, the weight of $w$ is the sum of weights of the derivation trees yielding $w$, and if $w\notin\sema{\aut{G}}$ then $\semagrmr{\grmr{W}}(w)=0$.
If the sum of all derivation trees in $\sema{\grmr{G}}$, namely $\sum_{w\in\sema{\grmr{G}}}\grmr{W}(w)$, is finite we say that $\aut{W}$ is \emph{convergent}. 
\subsubsection{Probabilistic Context Free Grammar}
A \emph{probabilistic context free grammar} (PCFG) is a WCFG 
$\grmr{P}=\tuple{\grmr{G},\theta}$ where $\grmr{G}=\langle \Vars,\Sigma,R,S\rangle$ is a CFG and $\theta:R\rightarrow [0,1]$ is a function mapping each production rule of $\grmr{G}$ to a weight in the range $[0,1]$ that satisfies:
\begin{equation*}
    \sum_{(V \derives \alpha_i) \in R} \theta(V\derives \alpha_i)=1
\end{equation*}
for every $V\in \Vars$.\footnote{Probabilistic grammars are sometimes called \emph{stochastic grammars (SCFGs)}.}

One can see that if $\grmr{P}$ is a PCFG then  the sum of all derivations equals $1$, thus $\grmr{P}$  is convergent.

It was shown by \cite{abney1999relating, smith2007weighted} that convergent WCFGs can be converted into PCFGs, hence an algorithm for learning convergent WCFGs can be used to learn PCFGs.

\subsection{Tree Automata}\label{sec:treeAutomata}
The definition of trees and tree automata makes use of the notion a \emph{ranked alphabet}. 
%\begin{defi}
A \emph{ranked alphabet} is a finite set of symbols $\Sigma=\bigcup_{k\in\mathbb{N}}\Sigma_{(k)}$ which is partitioned into pairwise disjoint subsets $\Sigma_{(k)}$. The symbols in $\Sigma_{(k)}$ are said to have rank $k$. We mark the rank of a symbol $\sigma$ by $\rank(\sigma)$.
%\end{defi}
A tree over a ranked alphabet $\Sigma$ is formally defined as follows:
%\begin{defi}
A \emph{tree domain} $\dom{t}$ over a ranked alphabet $\Sigma$ is a subset of $\mathbb{N}^{*}$ such that the following holds:
\begin{itemize}
    \item $\dom{t}$ is prefix-closed. That is, if $x\in\dom{t}$ and $y$ is a prefix of $x$, then $y\in\dom{t}$.
    \item If $x\cdot i\in\dom{t}$ for $i\in\mathbb{N}$ then $x\cdot j\in\dom{t}$ for every $j<i$.
\end{itemize}
An element of $\dom{t}$ is called a \emph{node} of $t$.
%\end{defi}
%\begin{defi}
A \emph{tree} is a mapping $t:\dom{t}\rightarrow\Sigma$ where $t(x)\in\Sigma_{(k)}$ if $k$ is the maximal element in $\mathbb{N}$ such that $x\cdot k\in\dom{t}$.
That is, a node labeled by $\sigma\in\Sigma{(k)}$ has $k$ children.
%\end{defi}
%
\begin{figure}
\vspace{-2cm}
\centering
\begin{minipage}{.25\textwidth}
\scalebox{0.75}{
    \begin{tikzpicture}
        \node[shape=circle,draw=none] (B1) at (0,3) {$S$};
        \node[shape=circle,draw=none] (B2) at (0,2) {$N_{1}$};
        \path [-] (B1) edge node[right] {} (B2);
        \node[shape=circle,draw=none] (B3) at (1,1) {$N_{1}$};
        \node[shape=circle,draw=none] (B4) at (-1,1) {$a$};
        \node[shape=circle,draw=none] (stam) at (-3,3) { };
        \path [-] (B2) edge node[right] {} (B3);
        \path [-] (B2) edge node[right] {} (B4);
        \node[shape=circle,draw=none] (B5) at (1,0) {$a$};
        \path [-] (B3) edge node[right] {} (B5);
    \end{tikzpicture}
    }
\end{minipage}%
\begin{minipage}{.75\textwidth}
\vspace{1cm}
\scalebox{0.75}{
    \begin{tikzpicture}
        \node[shape=circle,draw=none] (sigma) at (5,4) {$\Sigma=\{\ranked{\Sigma}{0}, \ranked{\Sigma}{1},\ranked{\Sigma}{2}\}$ where};
        \node[shape=circle,draw=none] (sigma) at (5,3) {$\ranked{\Sigma}{0}=\{a,b\},\ \ranked{\Sigma}{1}=\{S,N_{1}\},\ \ranked{\Sigma}{2}=\{N_{1}\}$};
        \node[shape=circle,draw=none] (dom) at (5,2) {$\dom{t}=\{\varepsilon,0,00,01,010\}$};
        \node[shape=circle,draw=none] (t) at (5,1) {$t(\varepsilon)=S,\ t(0)=N_{1},\ t(00)=a,\ t(01)=N_{1},\ t(010)=a$};
    \end{tikzpicture}}
\end{minipage}
\vspace{-2.5cm}
\caption{A tree $t$, and its corresponding ranked alphabet, and the domain $\dom{t}$.}
\label{fig:treeExample}
\end{figure}
An illustration of a tree over a ranked alphabet is given in Fig.\ref{fig:treeExample}.

The set of all trees over the ranked alphabet $\Sigma$ is denoted by $\trees(\Sigma)$. 
%\begin{defi}
A \emph{skeletal alphabet} is a ranked alphabet in which for every $k>0$ the set $\Sigma_{(k)}$ consists only of the special symbol $?$. Furthermore, $?\notin \Sigma_{{0}}$.
%\end{defi}
%\begin{defi}
Let $t\in\trees(\Sigma)$, the skeletal description of $t$, denoted by $\skel(t)$, is a tree with the same topology as $t$, in which the symbol in all internal nodes is $?$, and the symbols in all leaves are the same as in $t$.
%\end{defi}
%\begin{defi}
Let $T$ be a set of trees. The corresponding \emph{skeletal set}, denoted $\skels(T)$ is 
%\begin{equation*}
    $\skels(T)=\{\skels(t)~|~t\in T\}$.
%\end{equation*}
%\end{defi}
A tree language over a skeletal alphabet is called a \textit{skeletal tree language}.

We are now ready to define a bottom-up-finite-state tree automaton. % is defined as follows. %, as defined in \cite{drewes2007query}.
\begin{defi}
A \emph{bottom-up-finite-state tree automaton}, in short {FTA}, is a tuple $\aut{A}=(\Sigma,Q,\Delta,F)$ where:
\begin{itemize}
    \item $\Sigma$ is the ranked input alphabet
    \item $Q$ is the finite set of states
    \item $\Delta=\bigcup_{k=1}^{p} \Delta_{k}$ is the transition function, where $\Delta_{k}:Q^{k}\times \Sigma_{k}\rightarrow Q$ is the transition function for symbols of arity $k$.
    \item $F\subseteq Q$ is a set of accepting states.
\end{itemize}
\end{defi}
A tree language $L$ is called a \textit{regular tree language} if there exists an FTA $\aut{A}$ s.t $L=L(\aut{A})$.

An example for a tree automaton is available in Figure.\ref{fig:treeAutomaton}.
\begin{figure}[H]
    \centering
    \begin{minipage}{.45\textwidth}
        \vspace{-1cm}
        \scalebox{0.75}{
            \begin{tikzpicture}
                \node[shape=circle,draw=none] (auto) at (0,5) {$\mathcal{A}=\langle Q,\Sigma,\delta,F\rangle$};
                \node[shape=circle,draw=none] (states) at (0,4) {$Q=\{q_{0},q_{1}\},F=\{q_{0}\}$};
                \node[shape=circle,draw=none] (alphabet) at (0,3) {$\Sigma=\{\ \ranked{\Sigma}{0}=\{a,b\},\ \ranked{\Sigma}{2}=\{c\}\ \}$};
                \node[shape=circle,draw=none] (delta1) at (0,2) {$\Delta((),a)=q_{0},\ \Delta((),b)=q_{1}$};
                \node[shape=circle,draw=none] (delta2) at (0,1) {$\Delta((q_{0},q_{0}),c)=q_{0},\ \Delta((q_{0},q_{1}),c)=q_{0}$};
                \node[shape=circle,draw=none] (delta3) at (0,0) {$\Delta((q_{1},q_{0}),c)=q_{0},\ \Delta((q_{1},q_{1}),c)=q_{1}$};
            \end{tikzpicture}}
    \end{minipage}%
    \begin{minipage}{.20\textwidth}
        \vspace{-2cm}
        \begin{tikzpicture}
    	\newcommand*\Astate{$\textcolor{gray}{q_{0}}$}
    	\newcommand*\Adraw{gray}
    	\newcommand*\Bstate{$\textcolor{gray}{q_{1}}$}    
    	\newcommand*\Bdraw{gray}
    	\newcommand*\Cstate{$\textcolor{gray}{q_{0}}$}   
    	\newcommand*\Cdraw{gray}
    	\newcommand*\Dstate{$\textcolor{gray}{q_{0}}$}   
    	\newcommand*\Ddraw{gray}
    	\newcommand*\Estate{$\textcolor{gray}{q_{1}}$}  
    	\newcommand*\Edraw{gray} 
    	\foreach \i\j\n\label\state\offset\statedraw in {0/0/A/c/\Astate/1/\Adraw,-1/-1/B/b/\Bstate/-1/\Bdraw,1/-1/C/c/\Cstate/1/\Cdraw,0.5/-2/D/a/\Dstate/-1/\Ddraw,1.5/-2/E/b/\Estate/1/\Edraw}{
        	\node[shape=circle,draw=none] (\n) at (\i,\j) {\tiny{\label}};
        	\node[shape=circle,draw=\statedraw] (\n_2) at (\i+\offset,\j) {\tiny{\state}};
    	}
        \path [-] (A) edge node[above] {} (C);
        \path [-] (A) edge node[right] {} (B);
        \path [-] (C) edge node[above] {} (D);
        \path [-] (C) edge node[above] {} (E);
        \end{tikzpicture}
    \end{minipage}%
    \vspace{-1.5cm}
    \caption{\textbf{Left:} a tree automaton $A$ that accepts all trees which contain a leaf tagged with $a$. \textbf{Right:} a tree, annotated (in gray) by the states calculated by $A$ for each node of the tree.}
    \label{fig:treeAutomaton}
\end{figure}
\subsection{Multiplicity Automata}\label{sec:MA}
%\begin{defi}
A (word) automaton defines a function from words over $\Sigma$ to $\mathbb{B}=\{0,1\}$.
Often we are interested in function mapping words to a richer set of values.
Such functions are termed \emph{word series}.
A word series $L$ over a field $\mathbb{F}$ and an alphabet $\Sigma$ is a function $L:\Sigma^{*}\rightarrow\mathbb{F}$.
A multiplicity automaton is a machine that recognizes word series. Its formal definition follows.
%\end{defi}
\begin{defi}
A \emph{multiplicity word automaton}, in short MWA, is a tuple $M=\langle\mathbb{F}^{r},\Sigma,\lambda,\gamma,\mu\rangle$ where:
\begin{itemize}
\item $\mathbb{F}$ is some field, and $r\in\mathbb{N}$ is the dimension of $M$.
\item $\Sigma$ is a the alphabet.
\item $\lambda,\gamma\in\mathbb{F}^{r}$.
\item $\mu=\{\mu_{\sigma}:\sigma\in\Sigma\}$ where $\mu_{\sigma}\in\mathbb{F}^{r\times r}$ is an $r\times r$ matrix.
\end{itemize}
\end{defi}
The word-series of an MWA $M$ is $L_{M}$ and defined as follows:
\begin{equation*}
	L_{M}(w)=L_{M}(\sigma_{1}\sigma_{2}\hdots\sigma_{n})=\lambda\cdot\mu_{\sigma_{1}}\cdot\mu_{\sigma_{2}}\cdot\hdots\mu_{\sigma_{n}}\cdot\gamma^{\top}
\end{equation*}
\begin{exa}
Let $M=\langle \mathbb{R}^{2},\Sigma=\{a,b\},\lambda,\gamma,\mu\rangle$ be the following MWA:
\begin{center}
    \begin{tabular}{c c}
         $\lambda=\begin{bmatrix}1\\0\end{bmatrix}$ & $\gamma=\begin{bmatrix}0\\1\end{bmatrix}$  \\
         &\\
         $\mu_{a}=\begin{bmatrix}0&-1\\1&2\end{bmatrix}$ & $\mu_{b}=\begin{bmatrix}1&0\\0&1\end{bmatrix}$
    \end{tabular}
\end{center}
This word automaton calculates the number of $a$'s in a word. For example, for $w=\varepsilon$ we have:
\begin{equation*}
    L_{M}(\varepsilon)=\begin{bmatrix}1\\0\end{bmatrix}\cdot \begin{bmatrix}0&1\end{bmatrix}=0
\end{equation*}
And for $w=aba$ we have:
\begin{equation*}
    L_{M}(aba)=\begin{bmatrix}1\\0\end{bmatrix}\cdot \begin{bmatrix}0&-1\\1&2\end{bmatrix}\cdot\begin{bmatrix}1&0\\0&1\end{bmatrix}\cdot \begin{bmatrix}0&-1\\1&2\end{bmatrix} \begin{bmatrix}0&1\end{bmatrix}=2
\end{equation*}
\end{exa}


\subsection{Multiplicity Tree Automata}\label{sec:MTA}
\medskip
\subsubsection{Multilinear Functions}\label{subsec:multilinear}
\begin{defi}
A multilinear function $f:V_{1}\times V_{2}\times\hdots\times V_{k}\rightarrow W$ where $V_{1},V_{2},\hdots,V_{n},W$ are some vector spaces, is a function s.t. for each $i$, if all variables but $v_{i}$ are held constant, then $f(v_{1},\hdots,v_{i},\hdots,v_{k})$ is a linear function.
\end{defi}
For our purposes, we will assume from now on that $V_{1}=V_{2}=\hdots V_{k}=W$. That is, $f:W^{k}\rightarrow W$. If $W=\mathbb{R}^{n}$ we can describe $f$ using a $n^{k}\times n$ matrix.
\begin{equation*}
M_{f}=\begin{bmatrix} c^{1}_{11\hdots1} & c^{1}_{11\hdots 2} & \hdots & c^{1}_{nn\hdots n} \\
				    c^{2}_{11\hdots1} & c^{2}_{11\hdots 2} & \hdots & c^{2}_{nn\hdots n} \\
				    \vdots            &     \ddots         & \ddots &    \vdots          \\
				    c^{n}_{11\hdots1} & c^{n}_{11\hdots 2} & \hdots & c^{n}_{nn\hdots n} \\
	\end{bmatrix}
\end{equation*}
For $v_{1},v_{2},...,v_{k}\in W^{k}$, let $P_{v_{1},v_{2},...,v_{k}}\in\mathbb{R}^{n^{k}}$ be the following vector:
\begin{equation*}
P_{v_{1},v_{2},...,v_{k}}=\begin{bmatrix}v_{1}[1]\cdot v_{2}[1]\cdot\hdots v_{k}[1]\\ v_{1}[1]\cdot v_{2}[1]\cdot\hdots v_{k}[2]\\ \vdots \\ v_{1}[n]\cdot v_{2}[n]\cdot\hdots v_{k}[n]
						  \end{bmatrix}
\end{equation*}
Calculating $f(v_{1},v_{2},...,v_{k})$ is done in the following manner:
\begin{equation*}
	f(v_{1},v_{2},...,v_{k})=M_{f}\cdot P_{v_{1},v_{2},...,v_{k}}
\end{equation*}
\begin{exa}

For $W=\mathbb{R}^{2}$ let $\mu:W\times W\rightarrow W$ be the following multilinear function. Let $M_{\mu}$ be the following matrix:
\begin{equation*}
	M_{\mu}=\begin{bmatrix} 0& 1& 1& 0\\
						    0& 0& 0& 1\end{bmatrix}
\end{equation*}
For $v_{1}=\begin{bmatrix}2\\1\end{bmatrix}$ and $v_{2}=\begin{bmatrix}1\\2\end{bmatrix}$ we have:
\begin{equation*}
	P_{v_{1},v_{2}}=\begin{bmatrix}2\cdot 1\\2\cdot 2\\1\cdot 1\\1\cdot 2\end{bmatrix}=\begin{bmatrix}2\\4\\1\\2\end{bmatrix}
\end{equation*}
So:
\begin{equation*}
	\mu(v_{1},v_{2})=M_{\mu}\cdot P_{v_{1},v_{2}}=\begin{bmatrix}5\\2\end{bmatrix}
\end{equation*}
\end{exa}
\begin{defi}
A \emph{Multiplicity Tree Automaton (MTA)} is a tuple $M=\langle W=\mathbb{F}^{r},\Sigma,\lambda,\mu\rangle$ where:
\begin{itemize}
\item $W$ is a vector space, where $\mathbb{F}$ is some field, and $r\in\mathbb{N}$ is the dimension of $M$.
\item $\Sigma=\Sigma_{(0)}\cup\Sigma_{(1)}\cup\hdots\cup\Sigma_{(p)}$ is our ranked alphabet.
\item $\lambda\in\mathbb{F}^{r}$.
\item $\mu=\{\mu_{\sigma}:\sigma\in\Sigma\}$ where $\mu_{\sigma}:W^{k}\rightarrow W$ is a multilinear function, where $k$ is the arity of $\sigma$.
\end{itemize}
\end{defi}
For an MTA $M=\langle W=\mathbb{F}^{r},\Sigma,\lambda,\mu\rangle$ and a tree $t\in\trees(\Sigma)$, let $\mu(t)$ be defined recursively as follows:
\begin{equation*}
	\mu(t)=\begin{cases} 
   \mu_{\sigma} &\text {if } t=\sigma \text{ is a leaf }\\
   \mu_{\sigma}(\mu(t_{1}),\mu(t_{2}),\hdots,\mu(t_{p})) &\text {if } t=\sigma(t_{1},t_{2},...,t_{p}) \\
  \end{cases}
\end{equation*}
The tree-series of an MTA $M$ $L_{M}$ is defined as follows:
\begin{equation*}
	L_{M}(t)=\mu(t)\cdot\lambda^{\top}
\end{equation*}
\begin{exa}
Let $\Sigma=\Sigma_{0}\cup\Sigma_{2}$ with $\Sigma_{0}=\{a\}$ and $\Sigma_{2}=\{b\}$. We will define the following MTA $M=\langle\mathbb{R}^{2},\Sigma,\lambda,\mu\rangle$. Where:
\begin{center}
    \begin{tabular}{c c c}
         $\lambda=\begin{bmatrix}1\\0\end{bmatrix}$ & $\mu_{a}=\begin{bmatrix}1\\1\end{bmatrix}$  & $\mu_{b}=\begin{bmatrix}0&1&1&0\\0&0&0&1\end{bmatrix}$\\
    \end{tabular}    
\end{center}
\begin{figure}[H]
    \vspace{-1cm}
    \begin{tikzpicture}
	\newcommand*\Astate{$\begin{bmatrix}3\\1\end{bmatrix}$}
	\newcommand*\Adraw{none}
	\newcommand*\Bstate{$\begin{bmatrix}1\\1\end{bmatrix}$}    
	\newcommand*\Bdraw{none}
	\newcommand*\Cstate{$\begin{bmatrix}2\\1\end{bmatrix}$}   
	\newcommand*\Cdraw{none}
	\newcommand*\Dstate{$\begin{bmatrix}1\\1\end{bmatrix}$}   
	\newcommand*\Ddraw{none}
	\newcommand*\Estate{$\begin{bmatrix}1\\1\end{bmatrix}$}  
	\newcommand*\Edraw{none} 
	\foreach \i\j\n\label\state\offset\statedraw in {0/0/A/b/\Astate/1/\Adraw,-1/-1/B/a/\Bstate/-1/\Bdraw,1/-1/C/b/\Cstate/1/\Cdraw,0.5/-2/D/a/\Dstate/-1/\Ddraw,1.5/-2/E/a/\Estate/1/\Edraw}{
    	\node[shape=circle,draw=none] (\n) at (\i,\j) {\tiny{\label}};
    	\node[shape=circle,draw=\statedraw] (\n_2) at (\i+\offset,\j) {\tiny{\state}};
	}
    \path [-] (A) edge node[above] {} (C);
    \path [-] (A) edge node[right] {} (B);
    \path [-] (C) edge node[above] {} (D);
    \path [-] (C) edge node[above] {} (E);
    
    \node[shape=circle,draw=none] (finalVal) at (6, -1) {$L_{M}(t)=\begin{bmatrix}3\\1\end{bmatrix}\cdot\begin{bmatrix}1&0\end{bmatrix}=3$};
\end{tikzpicture}
    \caption{The calculation of this MTA on a tree}
    \label{fig:mta}
\end{figure}
The calculation of this MTA, which calculates the number of leaves in a given tree, on the tree $b(a,b(a,a))$ is available in Figure.\ref{fig:mta}.
\end{exa}


==> querylearning.tex <==
In our learning setting, we assume we are given a black box model - our oracle. This oracle can answer two types of queries, membership and equivalence queries. In a membership query, the learner gives a word to the oracle, and the oracle should return him whether the word is in the target language or not. In an equivalence query, the learner gives an hypothesis for the target language to the oracle. The oracle should return yes if the hypothesis is correct, in that case the algorithm terminates. Otherwise, it should return a counter-example, a word which the learner didn't tag correctly. The main scheme of the learning setting is available in Figure.\ref{fig:querylearningsetting}.

\begin{figure}
    \centering
    \begin{tikzpicture}
    	\newcommand*\mqstr{$w\in L$?}
    	\newcommand*\mqans{yes/no}
    	\newcommand*\eqstr{$L=\sema{G}$?}    
    	\newcommand*\eqans{yes/no\\ with counter example}
    	\node[shape=circle, draw=none] (Aup) at (1, 1.6) {};
    	\node[shape=circle, draw=none] (Aup2) at (1, 1.4) {};
    	\node[shape=circle, draw=none] (Adown) at (1, -1.4) {};
    	\node[shape=circle, draw=none] (Adown2) at (1, -1.6) {};
    	\node[shape=circle, draw=none] (Bup) at (5, 1.6) {};
    	\node[shape=circle, draw=none] (Bup2) at (5, 1.4) {};
    	\node[shape=circle, draw=none] (Bdown) at (5, -1.4) {};
    	\node[shape=circle, draw=none] (Bdown2) at (5, -1.6) {};
        \node[shape=rectangle,rounded corners,draw=black, minimum height=4cm, minimum width=2cm] (A) at (0,0) {Learner};
        \node[shape=rectangle,rounded corners,draw=black, minimum height=4cm, minimum width=2cm, align=center] (B) at (6.5,0) {Oracle -\\ Black box model};
            \path [->] (Aup) edge node[above] {\mqstr} (Bup);
            \path [->] (Bup2) edge node[below] {\mqans} (Aup2) ;
            \path [->] (Adown) edge node[above] {\eqstr} (Bdown);
            \path [->] (Bdown2) edge node[below, align=center] {\eqans} (Adown2) ;
    \end{tikzpicture}
    \caption{The learning setting}
    \label{fig:querylearningsetting}
\end{figure}


\subsection{Learning Regular Languages (L* algorithm)}\label{sec:lstar}
The algorithm that introduced this learning setting is \lstar \cite{Angluin87}. This algorithm learns a regular language from a black box model. The ideas used in this algorithm provide the basis for all algorithms who followed, including ours. The algorithm maintains two sets $S,E\subseteq\Sigma^{*}$. $S$ is a set of prefixes, and $E$ is a set of suffixes. In addition, the algorithm maintains a data-structure called the observation table. $T:(S\cup S\cdot\Sigma)\times E\rightarrow \{0,1\}$ such that:
\begin{equation*}
	T(s,e)=\begin{cases} 
   1 &\text {if } s\cdot e\in L\\
   0 &\text {if } s\cdot e\notin L \\
  \end{cases}
\end{equation*}
When filling the table, the algorithm uses membership queries, to decide whether $s\cdot e\in L$.
\begin{defi}
For a given $s\in S\cup S\cdot \Sigma$ we denote by $T[s]$ the row corresponding to $s$ in the table, that is:
\begin{equation*}
    T[s] = (T(s\cdot e_{1}),T(s\cdot e_{2}),\dots T(s\cdot e_{k})), E=\{e_{1},e_{2},\dots,e_{k}\}
\end{equation*}
\end{defi}
\begin{defi}
An observation table \emph{closed}, if for every $s\in S\cdot\Sigma$, there exists $s'\in S$ s.t.:
\begin{equation*}
    T[s] = T[s']
\end{equation*}
\end{defi}
\begin{defi}
A table $T$ is \emph{consistent} if for every $s_{1},s_{2}\in S$, s.t. $T[s_{1}]=T[s_{2}]$, and for every $\sigma\in\Sigma$, we have that $T[s_{1}\cdot\sigma]=T[s_{2}\cdot\sigma]$.
\end{defi}
Once an observation table is closed and consistent, the algorithm can extract an automaton $M=\langle Q,\Sigma,\delta,s,A\rangle$ from it, where:
\begin{itemize}
    \item $Q=\{T[s]:s\in S\}$
    \item $s=T[\varepsilon]$
    \item $A=\{T[s]\in Q: T[s][\varepsilon]=1\}$
    \item $\delta(T[s],\sigma)=T[s\cdot\sigma]$
\end{itemize}
In Figure.\ref{fig:observationTable} you can see a closed and consistent observation table, and the DFA extracted from it.

\begin{figure}
    \begin{minipage}{.4\textwidth}
        \begin{tabular}{ c|c|c|c } 
          & $\varepsilon$ & $a$ & $b$ \\ \hline
         \rowcolor{gray!50} $\varepsilon$ & $1$ & $1$ & $0$ \\ \hline
         \rowcolor{gray!50} $a$ & $1$ & $1$ & $0$ \\ \hline
         \rowcolor{gray!10}$b$ & $0$ & $0$ & $0$ \\  \hline
         \rowcolor{gray!50} $\boldsymbol{aa}$ & $1$ & $1$ & $0$ \\ \hline
         \rowcolor{gray!10} $\boldsymbol{ab}$ & $0$ & $0$ & $0$ \\ \hline
         \rowcolor{gray!10} $\boldsymbol{ba}$ & $0$ & $0$ & $0$ \\ \hline
         \rowcolor{gray!10} $\boldsymbol{bb}$ & $0$ & $0$ & $0$ \\ 
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \begin{tikzpicture} [->,auto,node distance=2.2cm,line width=0.2mm,initial text=]
        \tikzset{elliptic state/.style={draw,ellipse,minimum height=0.8cm}}
        \node[elliptic state, ellipse, initial, accepting, initial,inner sep=0pt,  fill=gray!50] (q1) {$\tiny\begin{bmatrix}1&1&0\end{bmatrix}$};
        \node[elliptic state, ellipse, below of=q1,inner sep=0pt, fill=gray!10] (q2) {$\tiny\begin{bmatrix}0&0&0\end{bmatrix}$};
        
        \draw (q1)  edge[loop right] node{$a$} (q1);
        \draw (q1)  edge[left] node{$b$} (q2);
        \draw (q2)  edge[loop right] node{$a,b$} (q2);
        \end{tikzpicture}
    \end{minipage}%
    \caption{A closed and consistent observation table, and the automaton extracted from it. The target language is $a^{*}$. The sets $S=E=\{\varepsilon,a,b\}$, the two different unique rows are highlighted with different shades of gray, the text for the rows that belong to $S\cdot\Sigma$ are marked with bold font.}
    \label{fig:observationTable}
\end{figure}
The main idea of the algorithm and its successors can be described as follows: Initialize the observation table in some deterministic way, in \lstar this is done by setting $S=E=\{\varepsilon\}$, then attempt to make the table closed and consistent. When the table satisfies these conditions, extract an automaton from it and ask an equivalence query. If the answer is positive terminate, otherwise use the counter example to extend the observation table. The entire pseudo-code of the algorithm is available in Figure.\ref{fig:lstar}.
\begin{figure}
    \centering
    \scalebox{0.8}{
        \begin{minipage}{0.55\textwidth}
        \begin{algorithm}[H]\label{algLstarClose}
        \caption{$L^{*}$ close}
        \begin{algorithmic}[H]
        \Procedure{make\_closed($T,S,E$)}{}
        \For {each $s\in\Sigma(S)$}
        \If {$T[s]\notin\{T[s']:s'\in S\}$}
        \State $S\gets S\cup\{s\}$
        \State Update $T$ using $\mq$
        \EndIf
        \EndFor
        \EndProcedure
        \end{algorithmic}
        \end{algorithm}
    \end{minipage}%
    }
    \scalebox{0.8}{
        \begin{minipage}{0.7\textwidth}
        \begin{algorithm}[H]\label{algLstarConsistent}
        \caption{$L^{*}$ consistent}
        \begin{algorithmic}[H]
        \Procedure{make\_consistent($T,S,E$)}{}
        \For {$s_{1},s_{2}\in S$ s.t. $T[s_{1}]=T[s_{2}]$}
        \For {$\sigma\in\Sigma,e\in E$}
        \If {$\mq(s_{1}\cdot\sigma\cdot e)\neq\mq(s_{2}\cdot\sigma\cdot e)$}
        \State $E\gets E\cup\{\sigma\cdot s\}$
        \State Update $T$ using $\mq$
        \EndIf
        \EndFor
        \EndFor
        \EndProcedure
        \end{algorithmic}
        \end{algorithm}
    \end{minipage}%
    }
    \begin{minipage}{1\textwidth}
        \begin{algorithm}[H]\label{algLstarMain}
        \caption{$L^{*}$ learn}
        \begin{algorithmic}[H]
        \Procedure{learn()}{}
        \State $S\gets\{\varepsilon\},E\gets\{\varepsilon\}$
        \State Fill $T$ using $\mq$
        \While {true}
        \While {$T$ isn't closed or $T$ isn't consistent}
        \State make\_closed($T,S,E$)
        \State make\_consistent($T,S,E$)
        \EndWhile
        \State $M\gets$ extract($T$)
        \State $c\gets\eq(M)$
        \If {$c=\text{null}$}
            \State return $M$
        \Else
            \State $S\gets S\cup\text{pref}(c)$
        \EndIf
        \EndWhile
        \EndProcedure
        \end{algorithmic}
        \end{algorithm}
    \end{minipage}
    \caption{Caption}\dana{hmmm}
    \label{fig:lstar}
\end{figure}


\subsection{Learning Regular Tree Languages}\label{sec:gstar}
Regular tree languages (modeled as FTAs) can also be learned using \mq\ and \eq\ \cite{sakakibara1990learning,drewes2007query} via an extension of Angluin's algorithm for regular languages. We will term this algorithm \gstar.
This algorithm also maintains an observation table like in the original \lstar, and assumes an oracle which can answer membership and equivalence queries on trees and tree-automata respectively.

The algorithm also attempts to make the observation table closed and consistent, and once it it closed and consistent it extracts a bottom up tree automaton from it.
Instead of the set $S$ of prefixes the algorithm maintains a set $S$ of trees. Since we can't concatenate two trees, instead of the set $E$ of suffixes the algorithm maintains a set $C$ of \emph{contexts}.

\subsubsection{Contexts}
\begin{defi}
Let $\Sigma$ be a ranked alphabet. a context is a tree over $\Sigma\cup\{\context\}$, where $\context$ is a symbol of arity $0$, and $\context\notin\Sigma_{0}$. A tree is a context if $\context$ appears in the tree exactly once.
\end{defi}
\begin{defi}
For a context $c$ and a tree $t$, we denote by $\contextConcat{c}{t}$ the tree obtained by replacing $\context$ in $c$ by $t$.
\end{defi}
\begin{figure}
    \centering
    \begin{minipage}{0.2\textwidth}
    \begin{tikzpicture}
    	\foreach \i\j\n\label in {0/0/A/c,-1/-1/B/b,1/-1/C/$\context$}{
        	\node[shape=circle,draw=none] (\n) at (\i,\j) {\small{\label}};
    	}
        \path [-] (A) edge node[above] {} (C);
        \path [-] (A) edge node[right] {} (B);
    \end{tikzpicture}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \begin{tikzpicture}
    	\foreach \i\j\n\label in {0/0/A/c,-1/-1/B/a,1/-1/C/b}{
        	\node[shape=circle,draw=none] (\n) at (\i,\j) {\small{\label}};
    	}
        \path [-] (A) edge node[above] {} (C);
        \path [-] (A) edge node[right] {} (B);
        \end{tikzpicture}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \begin{tikzpicture}
        	\foreach \i\j\n\label in {0/0/A/c,-1/-1/B/b,1/-1/C/c,0.5/-2/D/a,1.5/-2/E/b}{
            	\node[shape=circle,draw=none] (\n) at (\i,\j) {\small{\label}};
        	}
            \path [-] (A) edge node[above] {} (C);
            \path [-] (A) edge node[right] {} (B);
            \path [-] (C) edge node[above] {} (D);
            \path [-] (C) edge node[above] {} (E);
        \end{tikzpicture}
    \end{minipage}%
    \caption{A context $c$ on the left, a tree $t$ on the middle, and their concatenation $\contextConcat{c}{t}$ on the right }
    \label{fig:contextConcat}
\end{figure}
An example for a context, and the concatenation of a context to a tree is available in Figure.\ref{fig:contextConcat}.


\subsubsection{Converting Tree Automata to CFG}
It was shown by \cite{LEVY1978192, Sakakibara88} that the set of structural descriptions of a context free grammar constitute a regular tree language. The bottom up tree automaton for that regular tree language can be converted to a context free grammar.

Let $A$ be a tree automata s.t. $L(A)=\skel(\trees(\mathcal{G})))$ for some CFG $\mathcal{G}$.
$A=\langle Q,\Sigma,A,\delta,\rangle$ can be converted to $\mathcal{G}=\langle\Sigma,N,R,S\rangle$ in the following way:

\begin{itemize}
\item $N=Q\cup\{S\}$
\item $S\rightarrow q$ for every $q\in A$
\item $q_{i}\rightarrow q_{j_{1}}q_{j_{2}}\hdots q_{j_{p}}$ if $\delta(?,(q_{j_{1}},q_{j_{2}},\hdots,q_{j_{p}}))=q_{i}$
\item $q_{i}\rightarrow \sigma$ if $\Delta(\sigma)=q_{i}$
\end{itemize}
\begin{exa}
Let $\mathcal{A}=\langle Q,\Sigma,A,\Delta\rangle$ be the following tree automaton:
\begin{itemize}
    \item $Q=\{q_{0},q_{1},q_{2},q_{3}\}$
    \item $\Sigma=\{\Sigma_{0}=\{a,b\}, \Sigma_{2}=\{?\}, \Sigma_{3}=\{?\}\}$
    \item $A=\{q_{0}\}$
    \item $\delta(a,())=q_{1}$, $\delta(b,())=q_{2}$, $\delta(?,(q_{1},q_{2}))=q_{0}$, $\delta(?,(q_{1},q_{0},q_{2}))=q_{0}$ and for every other states tuple $T_{q}\in Q^{2}\cup Q^{3}$ we have that $\delta(?,T_{q})=q_{3}$ 
\end{itemize}
Applying the transformation we will obtain the following grammar:
\begin{align*}
    S&\rightarrow q_{0}\\
    q_{0}&\rightarrow q_{1}q_{0}q_{2}\mid q_{1}q_{2}\\
    q_{1}&\rightarrow a\\
    q_{2}&\rightarrow b\\
    q_{3}&\rightarrow q_{i}q_{j} (q_{i},q_{j})\in Q^{2}~|~ q_{i}q_{j}q_{k} (q_{i},q_{j},q_{k})\in Q^{3}
\end{align*}
We can describe this grammar more concisely by removing $q_{3}$ since it cannot be derived from $S$, and changing $q_{1}$ and $q_{2}$ to be $a$ and $b$ respectively. We obtain this grammar:
\begin{align*}
    S&\rightarrow q_{0}\\
    q_{0}&\rightarrow a q_{0}b\mid ab\\
\end{align*}
Whose language is $a^{n}b^{n}$ for $n\geq 1$.
\end{exa}
\subsection{Learning Multiplicity Automata}
\subsubsection{The Hankel Matrix}
All generalizations of \lstar\ are based on the following idea -- A word or a tree language/series can be represented by its Hankel Matrix. The Hankel Matrix is a matrix with infinite rows and infinite columns. The rows of the matrix correspond to an infinite enumeration of $\Sigma^{*}$ in the case of words, or $\trees(\Sigma)$ in the case of trees.
In the case of words, the columns of the matrix also correspond to an infinite enumeration of $\Sigma^{*}$, while in the case of trees, the columns correspond to an infinite enumeration of all contexts over $\Sigma$. 
One can notice, that the observation table maintained by \lstar and its generalizations is a finite sub-matrix of the infinite Hankel Matrix.

For a regular language $L$, the number of unique rows in the Hankel Matrix is finite, this follows easily from the Myhill-Nerode theorem \cite{10.1145/568438.568455, nerode58}. We can term those unique rows a \emph{base} for the matrix (Recall the states of the automaton extracted by \lstar, which correspond to unique rows in the observation table).

In the case of \lstar, and \gstar (that learn word-languages and tree-languages, resp.) rows that are not in the basis should be equal to rows in the basis. The rows of the basis correspond to the automaton states, and the equalities to other rows determines the transition relation. In Figure \ref{fig:hankelRegular} the Hankel Matrix for the language $a^{*}$ is shown, and the two unique rows are highlighted.

In the case of \mstar, the algorithm that learns MTA, which will be shown in the next section, rows not in the basis should be expressible as a linear combination of rows in the basis, and the linear combinations determines the weights of the extracted automaton. Figure \ref{fig:hankelWordSeries} shows the Hankel Matrix for the word-series that assigns to each word the number of $a$'s in the word, in this matrix the first two rows linearly span the entire matrix. Figure \ref{fig:hankelTreeSeries} shows the Hankel Matrix for the tree-series that assigns to each tree the number of leaves in the tree, the rows of this matrix are also linearly spanned by the first two rows.

\begin{figure}
    \centering
      \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    &$\varepsilon$ & $a$ & $b$ & $aa$ & $ab$ & $ba$  & $bb$ & $aaa$ & $aab$ & $\hdots$ \\ \hline
       \rowcolor{gray!50} $\varepsilon$ & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & $\hdots$\\ \hline
        \rowcolor{gray!50} $a$ & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & $\hdots$\\ \hline
        \rowcolor{gray!10} $b$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & $\hdots$\\ \hline
         \rowcolor{gray!50}$aa$ & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & $\hdots$\\ \hline 
        \rowcolor{gray!10}$ab$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & $\hdots$\\ \hline
        \rowcolor{gray!10}$ba$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & $\hdots$\\ \hline
        \rowcolor{gray!10}$bb$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & $\hdots$\\ \hline
        \rowcolor{gray!50} $aaa$ & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & $\hdots$\\ \hline
        \rowcolor{gray!10}$aab$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & $\hdots$\\ \hline
        $\vdots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\hdots$\\ 
  \end{tabular}
    \caption{A Hankel Matrix for the regular language $a^{*}$, the two unique rows are highlighted in green and yellow.}
    \label{fig:hankelRegular}
\end{figure}


\begin{figure}
    \centering
    \scalebox{.8}{
        \begin{tikzpicture}
        \node[
            draw=none] at (-0.5,0) {    \begin{tabular}{ c|c|c|c|c|c|c|c|c|c|c|c } 
      & $\varepsilon$ & $a$ & $b$ & $aa$ & $ab$ & $ba$ & $bb$ & $aaa$ & $aab$ & $aba$ & $\hdots$ \\ \hline
      $\varepsilon$ & $0$ & $1$ & $0$ & $2$ & $1$ & $1$ & $0$ & $3$ & $2$ & $2$ & $\ddots$ \\ \hline
      $a$ & $1$ & $2$ & $1$ & $3$ & $2$ & $2$ & $1$ & $4$ & $3$ & $3$ & $\ddots$ \\ \hline
      $b$ & $0$ & $1$ & $0$ & $2$ & $1$ & $1$ & $0$ & $3$ & $2$ & $2$ & $\ddots$ \\ \hline
      $aa$ & $2$ & $3$ & $2$ & $4$ & $3$ & $3$ & $2$ & $5$ & $4$ & $4$ & $\ddots$ \\ \hline
     $ab$ & $1$ & $2$ & $1$ & $3$ & $2$ & $2$ & $1$ & $4$ & $3$ & $3$ & $\ddots$ \\ \hline
     $ba$ & $1$ & $2$ & $1$ & $3$ & $2$ & $2$ & $1$ & $4$ & $3$ & $3$ & $\ddots$ \\ \hline
     $bb$ & $0$ & $1$ & $0$ & $2$ & $1$ & $1$ & $0$ & $3$ & $2$ & $2$ & $\ddots$ \\ \hline
     $aaa$ & $3$ & $4$ & $3$ & $5$ & $4$ & $4$ & $3$ & $6$ & $5$ & $6$ & $\ddots$ \\ \hline
     $\vdots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$\\  
    \end{tabular}};
            \node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center,anchor=center] at (7,2.5) {$v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center, anchor=center] at (7,1.8) {$v_{2}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center, anchor=center] at (7,1.1) {$v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.15\textwidth,
            align=center, anchor=center] at (7,0.4) {$2\cdot v_{2}-v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center, anchor=center] at (7,-0.3) {$v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center, anchor=center] at (7,-1) {$v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center, anchor=center] at (7,-1.7) {$v_{2}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.15\textwidth,
            align=center, anchor=center] at (7,-2.4) {$3\cdot v_{2}-2\cdot v_{1}$};
    \end{tikzpicture}}
    \caption{The Hankel Matrix for the word-series that returns the number of $a$'s in a word over the alphabet $\Sigma=\{a,b\}$. The first two rows linearly span the entire matrix. $H[\varepsilon]=v_{1}$ and $H[a]=v_{2}$. The rest of the rows can be described as a linear combination of $v_{1}$ and $v_{2}$.}
    \label{fig:hankelWordSeries}
\end{figure}


\begin{figure}
    \centering
    \scalebox{.8}{
    \begin{tikzpicture}
        \node[draw=none] at (0,0) {\begin{tabular}{ c|c|c|c|c|c } 
  & $\context$ & \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$\context$}};
 \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A);
 \path [-] (root) edge node[above] {} (A2);
 \end{tikzpicture} & \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$\context$}};
 \path [-] (root) edge node[above] {} (A);
 \path [-] (root) edge node[above] {} (A2);
 \end{tikzpicture} & \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,2) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A1) at (0,1) {\tiny{$\context$}};
 \node[shape=circle,draw=none] (B1) at (1,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A2) at (1.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A3) at (0.5,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A1);
 \path [-] (root) edge node[above] {} (B1);
 \path [-] (B1) edge node[above] {} (A2);
 \path [-] (B1) edge node[above] {} (A3);
 \end{tikzpicture}&$\hdots$\\ \hline
 
 $a$ & $1$ & $2$ & $2$ & $3$ &$\ddots$\\ \hline
 
 \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A);
 \path [-] (root) edge node[above] {} (A2);
 \end{tikzpicture} & $2$ & $3$ & $3$ & $4$ &$\ddots$ \\  \hline
 \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,2) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A1) at (0,1) {\tiny{$a$}};
 \node[shape=circle,draw=none] (B) at (1,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A2) at (0.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A3) at (1.5,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A1);
 \path [-] (root) edge node[above] {} (B); 
 \path [-] (B) edge node[above] {} (A2);
 \path [-] (B) edge node[above] {} (A3);
 \end{tikzpicture} & $3$ & $4$ & $4$ & $5$ &$\ddots$\\  \hline
 \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,2) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A1) at (1,1) {\tiny{$a$}};
 \node[shape=circle,draw=none] (B) at (0,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A2) at (-0.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A3) at (0.5,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A1);
 \path [-] (root) edge node[above] {} (B); 
 \path [-] (B) edge node[above] {} (A2);
 \path [-] (B) edge node[above] {} (A3);
 \end{tikzpicture} & $3$ & $4$ & $4$ & $5$ &$\ddots$ \\  \hline
 \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0,2) {\tiny{$b$}};
 \node[shape=circle,draw=none] (B1) at (1,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (B2) at (-1,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A1) at (1.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A2) at (0.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A3) at (-1.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A4) at (-0.5,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (B1);
 \path [-] (root) edge node[above] {} (B2); 
 \path [-] (B1) edge node[above] {} (A1);
 \path [-] (B1) edge node[above] {} (A2);
 \path [-] (B2) edge node[above] {} (A3);
 \path [-] (B2) edge node[above] {} (A4);
 \end{tikzpicture} & $4$ & $5$ & $5$ & $6$ &$\ddots$ \\ \hline
  $\vdots$ & $\ddots$ & $\ddots$ & $\ddots$ & $\ddots$ &$\ddots$\\ 
\end{tabular}};
\node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center,anchor=center] at (8,3.9) {$v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.1\textwidth,
            align=center, anchor=center] at (8,2.7) {$v_{2}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.15\textwidth,
            align=center, anchor=center] at (8,0.7) {$2\cdot v_{2}-v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.15\textwidth,
            align=center, anchor=center] at (8,-2.2) {$2\cdot v_{2}-v_{1}$};
            \node[draw=black,text=black,fill=gray!30,text width=0.15\textwidth,
            align=center, anchor=center] at (8,-5) {$3\cdot v_{2}-2\cdot v_{1}$};
    \end{tikzpicture}
    }
    \caption{The Hankel Matrix for the tree-series that returns the number of leaves in a tree over the ranked alphabet $\Sigma=\{\Sigma_{0}=\{a\},\Sigma_{2}=\{b\}\}$. The first two rows linearly span the entire matrix. $H[a]=v_{1}$ and $H[b(a,a)]=v_{2}$. The rest of the rows can be described as a linear combination of $v_{1}$ and $v_{2}$.}
    \label{fig:hankelTreeSeries}
\end{figure}
\subsubsection{Learning Multiplicity Tree Automata}\label{sec:mstar}
An algorithm for learning multiplicity tree automata, to which we refer as \mstar, was developed in~\cite{habrard2006learning}.\footnote{Following a learning algorithm developed for multiplicity word automata~\cite{BergadanoV96,BeimelBBKV00}.}

The algorithm maintains a set $T$ of trees, a set $B\subseteq T$ of trees called the base or hierarchical generator, and a set of contexts $C$. Like in the original \lstar, the algorithm maintains an observation table $H:(T\times C)\rightarrow\mathbb{K}$. 
\begin{defi}
Let $t\in T$. The vector $H[t]$ is defined as follows:
\begin{equation*}
    H[t] = \begin{bmatrix}
    H(t,c_{1})& H(t,c_{2})& \dots& H(t,c_{k})
    \end{bmatrix}, C=\{c_{1},c_{2},\dots,c_{k}\}
\end{equation*}
\end{defi}
\begin{defi}
Let $A\subseteq T$, $A=\{a_{1},a_{2},\dots,a_{m}\}$. The matrix $\hat{A}$ is defined as follows:
\begin{equation*}
    \hat{A}=   \begin{bmatrix}
           \vert & \vert & & \vert\\
           H[a_{1}] & H[a_{2}] & ... & H[a_{m}]\\
           \vert & \vert & & \vert
         \end{bmatrix}\\
\end{equation*}
\end{defi}
\begin{defi}
A set $B$ is an hierarchical generator if the following holds:
\begin{itemize}
    \item The set $B$ is minimal, that is -- each $b_{i}\in B$ is linearly independent of the rest. 
    \item $B$ is prefix closed, that is if $\sigma (e_{1},e_{2},\dots,e_{p})$ then $e_{i_{j}}\in B$ for $j=1,2,\dots,p$.
\end{itemize}
\end{defi}
\begin{defi}
An observation table is termed \emph{closed} if for every $t\in T$, $H[t]$ depends linearly on $B$. That is, there exists a vector $\alpha\in\mathbb{K}^{|B|}$ s.t. 
\begin{equation*}
    H[t]=\hat{B}\cdot\alpha
\end{equation*}
\end{defi}
Given a closed observation table, we can extract an MTA $M=\langle V,\mu,\lambda\rangle $ from it, in the following way:
\begin{itemize}
    \item $d=|B|$, $V=\mathbb{K}^{d}$
    \item $\lambda[i]=H(b_{i},\context)$.
    \item For every $t=\sigma(b_{i_{1}},b_{i_{2}},\dots,b_{i_{p}})$, let $\alpha_{t}$ be the vector s.t. $H[t]=\hat{B}\cdot\alpha$, set $\mu^{\sigma}_{i,i_{1},i_{2},\dots,i_{p}}$ to be $\alpha[i]$.
\end{itemize}
\begin{defi}
An observation table is termed consistent if for every $t,c\in T\times C$ we have that $H[t,c]=M(\contextConcat{t}{c})$. Where $M$ is the MTA extracted from the table.
\end{defi}
\begin{exa}
An example for an observation table, for the tree-series which assigns to each tree the number of leaves in it, is available in Figure.\ref{fig:mta_extract}. The ranked alphabet in this example is $\Sigma_{0}=\{a\}$, and $\Sigma_{2}=\{b\}$.

\begin{figure}
    \centering
\scalebox{.8}{
    \begin{minipage}{0.75\textwidth}
        \begin{tabular}{ c|c|c|c|c } 
  && $\context$ & \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$\context$}};
 \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A);
 \path [-] (root) edge node[above] {} (A2);
 \end{tikzpicture} & \begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$\context$}};
 \path [-] (root) edge node[above] {} (A);
 \path [-] (root) edge node[above] {} (A2);
 \end{tikzpicture} \\ \hline
 
 \cellcolor{red!50} $v_{1}$&$a$ & \cellcolor{purple!50} $1$ & $2$ & $2$ \\ \hline
 
 \cellcolor{orange!50} $v_{2}$&\begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A) at (0,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A2) at (1,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A);
 \path [-] (root) edge node[above] {} (A2);
 \end{tikzpicture} & \cellcolor{purple!50} $2$ & $3$ & $3$ \\  \hline
 \cellcolor{yellow!50} $2\cdot v_{2}-v_{1}$&\begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,2) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A1) at (0,1) {\tiny{$a$}};
 \node[shape=circle,draw=none] (B) at (1,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A2) at (0.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A3) at (1.5,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A1);
 \path [-] (root) edge node[above] {} (B); 
 \path [-] (B) edge node[above] {} (A2);
 \path [-] (B) edge node[above] {} (A3);
 \end{tikzpicture} & $3$ & $4$ & $4$ \\  \hline
 \cellcolor{green!50} $2\cdot v_{2}-v_{1}$&\begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0.5,2) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A1) at (1,1) {\tiny{$a$}};
 \node[shape=circle,draw=none] (B) at (0,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A2) at (-0.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A3) at (0.5,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (A1);
 \path [-] (root) edge node[above] {} (B); 
 \path [-] (B) edge node[above] {} (A2);
 \path [-] (B) edge node[above] {} (A3);
 \end{tikzpicture} & $3$ & $4$ & $4$ \\  \hline
 \cellcolor{blue!40} $3\cdot v_{2}-2\cdot v_{1}$&\begin{tikzpicture}
 \node[shape=circle,draw=none] (root) at (0,2) {\tiny{$b$}};
 \node[shape=circle,draw=none] (B1) at (1,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (B2) at (-1,1) {\tiny{$b$}};
 \node[shape=circle,draw=none] (A1) at (1.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A2) at (0.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A3) at (-1.5,0) {\tiny{$a$}};
 \node[shape=circle,draw=none] (A4) at (-0.5,0) {\tiny{$a$}};
 \path [-] (root) edge node[above] {} (B1);
 \path [-] (root) edge node[above] {} (B2); 
 \path [-] (B1) edge node[above] {} (A1);
 \path [-] (B1) edge node[above] {} (A2);
 \path [-] (B2) edge node[above] {} (A3);
 \path [-] (B2) edge node[above] {} (A4);
 \end{tikzpicture} & $4$ & $5$ & $5$\\ 
\end{tabular}
    \end{minipage}%
    \begin{minipage}{0.15\textwidth}
    \begin{align*}
        \mu_{a}=&\begin{bmatrix}&\cellcolor{red!50}1&\\&\cellcolor{red!50}0&\end{bmatrix}\\
        \mu_{b}=&\begin{bmatrix}&\cellcolor{orange!50}0&\cellcolor{yellow!50}-1&\cellcolor{green!50}-1&\cellcolor{blue!40}-2&\\&\cellcolor{orange!50}1&\cellcolor{yellow!50}2&\cellcolor{green!50}2&\cellcolor{blue!40}3&\end{bmatrix}\\
        \lambda=&\begin{bmatrix}&\cellcolor{purple!50}1&\\&\cellcolor{purple!50}2&\end{bmatrix}
    \end{align*}
    \end{minipage}%
    }
    \caption{A closed observation table (on the left) and the MTA extracted from it on the right. The base here is the first two rows, and as can be seen they linearly span the other rows of the table. The coefficients with which they span the table appear on the left-most column.}
    \label{fig:mta_extract}
\end{figure}
\end{exa}
